ChemFM as a Scaling Law Guided Foundation Model Pre-trained on Informative Chemicals

Traditional AI methods often rely on task-specific model designs and training, which constrain both the scalability of model size and generalization across different tasks. Here, we introduce ChemFM, a large foundation model specifically developed for chemicals. By conducting a series of scaling experiments, we identify UniChem as the informative molecular database for pre-training the foundation model. ChemFM comprises 3 billion parameters and is pre-trained on 178 million molecules using self-supervised causal language modeling to extract generalizable molecular representations. This model can be adapted to diverse downstream chemical applications using either full-parameter or parameter-efficient fine-tuning methods. ChemFM consistently outperforms state-of-the-art task-specific AI models across all tested tasks. Notably, it achieves up to 67.48% performance improvement across 34 property prediction benchmarks, up to 33.80% reduction in mean average deviation between conditioned and actual properties of generated molecules in conditional molecular generation tasks, and up to 3.7% top-1 accuracy improvement across 4 reaction prediction datasets. Moreover, ChemFM demonstrates its superior performance in predicting antibiotic activity and cytotoxicity, highlighting its potential to advance the discovery of novel antibiotics. Furthermore, we demonstrate that, as a foundation model, ChemFM exhibits strong data efficiency, requiring significantly fewer labeled training samples to achieve state-of-the-art performance. We anticipate that ChemFM will significantly advance chemistry research by providing a foundation model capable of effectively generalizing across a broad range of tasks with minimal additional training.

==> appendices.tex <==
\begin{appendices}
	\section{Section title of first appendix}\label{secA1}
\end{appendices}

==> conclusion.tex <==
\section{Conclusion}\label{sec13}


==> extended_figs_and_tables.tex <==

%
%
%
%\makeatletter
%\newcommand\formatlabel[1]{%
%	\noexpandarg
%	\IfSubStr{#1}{.}{%
%		\StrBefore{#1}{.}[\firstcaption]%
%		\StrBehind{#1}{.}[\secondcaption]%
%		\textbf{\firstcaption.} \secondcaption}{%
%		#1}%
%}
%\patchcmd{\@caption}{#3}{\formatlabel{#3}}
%\makeatother

\section*{Extended Data Figures and Tables}\label{sec:extended_data_figures_tables}

\makeatletter
\renewcommand{\tablename}{Extended Data Table \@gobble}
\renewcommand{\figurename}{Extended Data Fig. \@gobble}
\makeatother

% pretrain
%\input{tables/model_architecture_scaling_law}
%%\newpage
%\input{figures/scaling_law}
%\newpage

%\input{tables/lora_list}
%\newpage
%
% fine-tune
%% property_prediction
%\input{tables/dataset_moleculenet}
%\newpage
%\input{tables/results_PropPred}
%
%%\newpage
%%\input{tables/PropPred_config}
%
%\newpage
%\input{tables/results_PropPred_moleculenet_attentivefp}
%\newpage
%\input{tables/results_PropPred_moleculenet_molebert}
%
%
%%
%%
%%%\newpage
%%%\input{tables/dataset_admet}
%\newpage
%\input{tables/results_PropPred_Admet}
%
%
%%%\newpage
%%\input{tables/PropPred_config_admet}
%%\newpage
%%\input{tables/excluded_methods_admet}
%\newpage
%\input{tables/results_PropPred_Admet_wo_pre_training}
%\newpage
%\input{tables/results_PropPred_moleculenet_on_different_pretraining_data}
%
%\newpage
%\input{tables/additional_property_prediction}
%
%\newpage
%\input{figures/antibiotics}

%\input{tables/model_architecture}
%\newpage
%\newpage
%\input{tables/dataset_uspto}

%\input{figures/finetune_dataset}

%\newpage
%\input{tables/results_cond_mol_generation}
%
%\newpage
%\input{tables/results_cond_mol_generation_scaffold}
%%\newpage
%%\input{tables/results_cond_mol_generation_scaffold_2d}
%
%\newpage
%\input{figures/results_mol_gen_prop_distribution_1d}
%
%\newpage
%\input{figures/results_mol_gen_prop_distribution}
%
%\newpage
%\input{figures/results_mol_gen_scaffold_prop_distribution_1d}
%
%\newpage
%\input{figures/results_mol_gen_scaffold_prop_distribution}

%\newpage
%\input{tables/results_reaction_detail}

%\newpage
%\input{figures/data_efficient}

==> figures/benchmark_pretrain.tex <==
%
% 
\newcommand{\D}{6} % number of dimensions (config option)
\newcommand{\U}{5} % number of scale units (config option)
%%
\newdimen\R % maximal diagram radius (config option)
\R=1.5cm 
\newdimen\L % radius to put dimension labels (config option)
\L=2.0cm
\newcommand{\calangle}{360/\D+30} % calculated angle between dimension axes 

\definecolor{c1}{HTML}{af58ba}
\definecolor{c2}{HTML}{009ade}
\definecolor{c3}{HTML}{5E9432}

\definecolor{c4}{HTML}{f28522}
\definecolor{c5}{HTML}{ff1f5b}



%	\def\twodimlist{{{0.6, 0.8, 1.0}, {0.6, 0.8, 1.0}, {0.6, 0.8, 1.0}, {0.0, 0.1, 0.2},
%			{0.0, 0.2, 0.4}, {0.6, 0.8, 1.0}, {0.6, 0.8, 1.0}, {0.6, 0.8, 1.0},
%			{0.8, 0.6, 0.4}, {1.2, 1.0, 0.8}, {0.8, 0.6, 0.4}, {1.6, 1.1, 0.6}}}

	\def\chemfm{{ 1.000, 0.558, 0.993, 0.896, 0.896, 0.996}}
	
	
	%\path (0:3cm) coordinate (O); % define coordinate for origin
\begin{scope}[shift={(12.8, 3.2)}]
	% draw the spiderweb
	\foreach \X in {1,...,\D}{
		\pgfmathsetmacro{\value}{3.5/3}
		\draw (\X*\calangle:0) -- (\X*\calangle:\R);
		%\draw[dashed] (\X*\calangle:0) -- (\X*\calangle:1.1666);
	}
	
	% print the label
	\foreach \Y in {1,...,\U}{
		\foreach \X in {1,...,\D}{
			\path (\X*\calangle:\Y*\R/\U) coordinate (D\X-\Y);
			\fill (D\X-\Y) circle (1pt);
		}
		\draw [opacity=0.3] (30:\Y*\R/\U) \foreach \G in {1,...,\D}{
			-- (D\G-\Y)
		} -- cycle;
	}
	
	% define labels for each dimension axis (names config option)
	\path (1*\calangle:\L-0.2cm) node[align=center,font=\tiny] (L1) {Uniqueness};	
	\path (2*\calangle:\L) node[align=center,font=\tiny] (L2) {Novelty};
	\path (3*\calangle:\L) node[align=center,font=\tiny] (L3) {KLDiv};
	\path (4*\calangle:\L-0.2cm) node[align=center,font=\tiny] (L4) {$\text{IntDiv}_1$};
	\path (5*\calangle:\L) node[align=center,font=\tiny] (L5) {$\text{IntDiv}_2$};
	\path (6*\calangle:\L) node[align=center,font=\tiny] (L6) {Validity};
	
	\foreach \i in {1,...,\D} {
		\pgfmathsetmacro{\value}{\chemfm[\i-1]}
%		\pgfmathsetmacro{\xi}{\twodimlist[\i-1][0]}
%		\pgfmathsetmacro{\xo}{\twodimlist[\i-1][2]}
%		\pgfmathsetmacro{\ratio}{(\value-\xi)/(\xo-\xi)*0.6666+0.3333}
		\path (\i*\calangle:\R*\value) coordinate (data\i);
		%\coordinate (data\i) at (\i*\calangle:\R*\ratio) node (){\tiny {\ratio}}; % Replace this with your actual point calculation
	}	
	
	\draw [color=c5, fill=c5, line width=1pt, opacity=0.3]
	(data1) -- (data2) -- (data3) -- (data4) --
	(data5) -- (data6) --cycle;
	
	
	
\end{scope}

==> figures/benchmark_pretrain_bar.tex <==
\begin{axis}[
	%title={Performance Comparison}, 
	ylabel={AUC-PRC $\uparrow$},
	xmin=-0.00, xmax=12.00, 
	ymin=-0.00, ymax=1.0,
	width=0.80\textwidth,
	height=0.3\textwidth,
	clip=false,
	x tick label style={align=center, text width=1.5cm},
	xtick style={draw=none},
	every axis plot/.append style={
		ybar,
		bar width=18pt,
		bar shift=0pt,
		fill
	},
	nodes near coords={
		\pgfmathprintnumber[zerofill, precision=3]{\pgfplotspointmeta}
	},
	nodes near coords style={font=\scriptsize},
	xtick={1.5, 4.5, 7.5, 10.5},
	xticklabels={Antibiotics\\activity, HepG2\\cytotoxicity, HSkMC\\cytotoxicity, IMR-90\\cytotoxicity},
	ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
	yticklabels={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
	%xtick=\empty,
	legend style={at={(1,1)}, anchor=north east, legend columns=1, /tikz/every even column/.append style={column sep=0.5cm}}, % Legend at top right
	legend cell align={left},
	legend image code/.code={
		\draw [#1] (0cm,-0.15cm) rectangle (0.2cm,0.25cm);},
	]
	\addplot[ybar,blue]coordinates{(1.1,0.364)}; \addlegendentry{Chemprop\cite{dmpnn}};
	\addplot[ybar,red]coordinates{(1.9,0.613)}; \addlegendentry{ChemFM-1B};
	
	\addplot[ybar,blue]coordinates{(4.1,0.176)}; %\addlegendentry{MMNB\cite{MMNB}};
	\addplot[ybar,red]coordinates{(4.9,0.496)}; %\addlegendentry{ChemFM-1B};
	
	\addplot[ybar,blue]coordinates{(7.1,0.168)}; %\addlegendentry{MMNB\cite{MMNB}};
	\addplot[ybar,red]coordinates{(7.9,0.474)}; %\addlegendentry{ChemFM-1B};
	
	\addplot[ybar,blue]coordinates{(10.1,0.335)}; %\addlegendentry{MMNB\cite{MMNB}};
	\addplot[ybar,red]coordinates{(10.9,0.405)}; %\addlegendentry{ChemFM-1B};
	\node[anchor=north west, font=\small] at (rel axis cs:-0.1,1.1) {\textbf{e}};	
\end{axis}

==> figures/conditional_generation.tex <==
\begin{scope}[shift={(0.05,0.3)}]

%		%% molecular generation
		\node[draw=none, fill=color_molecular_generation_bg, rounded corners=6.0, minimum width=15.9cm, minimum height=4cm, opacity=0.3, anchor=north west] (molecular_generation) at (0, 4) {};
		\node[anchor=north west] at (molecular_generation.north west) {\small \bfseries b\, \small \ttfamily \bfseries Conditional Molecular Generation};
		
		
		\node[anchor=base] (icon1) at (0.25, 2.80) {\includegraphics[height=1em]{./figures/main_fig_elements/think_emoji}};
		\node[anchor=base, right=-1mm of icon1, align=left, text width=12cm, yshift=-0.2cm] (text) at (icon1.east) {\fontsize{6.5}{7.5}\selectfont
		\baselineskip=3pt
		Generating molecules that meet the following conditions \\
		1. Contain the specific scaffold: \\
		\\
		\\
		\\
		2. Number of hydrogen bond acceptors (HBA) is $4$ \\
		3. Quantitative estimate of drug-likeness (QED) is $0.60$ \\
		4. Synthetic accessibility score (SAS) is $3.06$
		\par};
		
		\node[anchor=base, right=-20mm of text, yshift=2mm] (icon2) at (6.05, 2.90) {\includegraphics[height=2.8em,page=1]{./figures/main_fig_elements/scaffold.pdf}};	
		
		
		\node[draw, fill=color_chemFM, text centered, rounded corners, minimum width=12.5cm, minimum height=0.8cm, align=center] (ChemFM-MG) at (8.0 , 1.5) {\footnotesize ChemFM};
		
		%scaffold
		\foreach \token [count=\i] in {c,1,c,n,c,n,c,1} {
			\node[rectangle, draw, fill=none,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-MG.south) + (\i*0.35 -5.93, -0.4cm)$) (token-\i) {\token};
			\draw[-stealth] (token-\i.north) -- ([xshift=0cm]token-\i.north |- ChemFM-MG.south);
		}
		\node[draw=myblue, rectangle, fill=none, left=of token-1, xshift=0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-scaffold) {\textcolor{myblue}{\textsc{Scaf}}};
		\draw[-stealth] (token-scaffold.north) -- ([xshift=0cm]token-scaffold.north |- ChemFM-MG.south);
		
		% aromatic ring
		\node[draw=myblue, rectangle, fill=none, right=of token-8, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-arom) {\textcolor{myblue}{\textsc{HBA}}};
		\draw[-stealth] (token-arom.north) -- ([xshift=0cm]token-arom.north |- ChemFM-MG.south);
		\node[draw=myred, rectangle, fill=none, right=of token-arom, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-c1) {\textcolor{myred}{\textsc{C4}}};
		\draw[-stealth] (token-c1.north) -- ([xshift=0cm]token-c1.north |- ChemFM-MG.south);
		
		% QED
		\node[draw=myblue, rectangle, fill=none, right=of token-c1, xshift=-0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-qed) {\textcolor{myblue}{\textsc{QED}}};
		\draw[-stealth] (token-qed.north) -- ([xshift=0cm]token-qed.north |- ChemFM-MG.south);
		
		\node[draw, rectangle, rounded corners=0.2em, right=of token-qed, xshift=-0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt, fill=Cyan!20] (token-mlp) {\textsc{MLP}};
		\draw[-stealth] (token-mlp.north) -- ([xshift=0cm]token-mlp.north |- ChemFM-MG.south);
		\draw[-stealth] ($(token-mlp.south)+(0.0, -0.3)$) -- (token-mlp.south) node[midway, below, font=\footnotesize, yshift=-0.4mm] {$0.60$};
		
		
		% SAS
		\node[draw=myblue, rectangle, fill=none, right=of token-mlp, xshift=-0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-sas) {\textcolor{myblue}{\textsc{SAS}}};
		\draw[-stealth] (token-sas.north) -- ([xshift=0cm]token-sas.north |- ChemFM-MG.south);
		
		\node[draw, rounded corners=0.2em, rectangle, fill=Cyan!20, right=of token-sas, xshift=-0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-mlp2) {{\textsc{MLP}}};
		\draw[-stealth] (token-mlp2.north) -- ([xshift=0cm]token-mlp2.north |- ChemFM-MG.south);
		\draw[-stealth] ($(token-mlp2.south)+(0.0, -0.3)$) -- (token-mlp2.south) node[midway, below, font=\footnotesize, yshift=-0.4mm] {$3.06$};
		
		% EOS
		\node[draw=myred, rectangle, fill=none, right=of token-mlp2, xshift=-0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-eos) {\textcolor{myred}{\textsc{EOS}}};
		\draw[-stealth] (token-eos.north) -- ([xshift=0cm]token-eos.north |- ChemFM-MG.south);
		
		
		\foreach \token [count=\i] in {C,S,c,1,n,c,n,c, $($, S, C, $)$,c,$1$,Br} {
			\node[rectangle, draw, fill=color_activate_token,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-MG.north) + (\i*0.35 + 0.30, +0.4cm)$) (token-\i) {\token};
			\draw[-stealth] ([xshift=0cm]token-\i.south |- ChemFM-MG.north) -- (token-\i.south);
		}
		\node[draw=myred, rectangle, fill=color_activate_token, right=of token-15, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-16) {\textcolor{myred}{\textsc{EOS}}};
		\draw[-stealth]([xshift=0cm]token-16.south |- ChemFM-MG.north) -- (token-16.south);
		
		% legends
		\node[draw=myblue, rectangle, fill=none, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-scaffold) at (9.5 , 3.7) {\textcolor{myblue}{\textsc{Scaf}}};
		\node[draw=myblue, rectangle, fill=none, right=of token-scaffold, xshift=-0.8cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-arom) {\textcolor{myblue}{\textsc{HBA}}};
		\node[draw=myblue, rectangle, fill=none, right=of token-arom, xshift=-0.8cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-qed2) {\textcolor{myblue}{\textsc{QED}}};
		\node[draw=myblue, rectangle, fill=none, right=of token-qed2, xshift=-0.8cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-sas2) {\textcolor{myblue}{\textsc{SAS}}};
		
		\node[draw=none, rectangle, fill=none, right=of token-sas2, xshift=-1.0cm, minimum height=0.3cm, minimum width=0.3cm, inner sep=1pt, outer sep=0pt] (token-script1) {\fontsize{6.5}{7.5} \selectfont Property identification token};
		
		\node[draw=myred, rectangle, fill=none, below=of token-sas2, xshift=0cm, yshift=+0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-c4) {\textcolor{myred}{\textsc{C4}}};
		\node[draw=none, rectangle, fill=none, below=of token-script1, yshift=+0.9cm, xshift=-0.45cm, minimum height=0.3cm, minimum width=5cm, inner sep=1pt, outer sep=0pt, align=left] (token-script2) {\fontsize{6.5}{7.5} \selectfont Category index token};
		\node[draw, rounded corners=0.2em, rectangle, fill=Cyan!20, below=of token-c4, yshift=+0.9cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-mlp3) {{\textsc{MLP}}};
		\node[draw=none, rectangle, fill=none, below=of token-script2, xshift=0.5cm, yshift=+0.9cm, minimum height=0.3cm, minimum width=5cm, inner sep=1pt, outer sep=0pt, align=left] (token-script3) {\fontsize{6.5}{7.5} \selectfont Shared value embedding layer};
		
		
		%($(mlp.north)+(-0.2, 0.0) $ ) -- ($(mlp.north) + (-0.2, 0.25)$ ) node[midway, above, font=\footnotesize, yshift=0.5mm] {$0$};
		
%		\node[draw=myred, rectangle, fill=none, right=of token-15, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-16) {\textcolor{myred}{\textsc{EOS}}};
%		\draw[-stealth] (token-16.north) -- ([xshift=0cm]token-16.north |- ChemFM-MG.south);
%		
%		\foreach \token [count=\i] in {C,C,1,C,O,1} {
%			\node[rectangle, draw, fill=color_activate_token,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-MG.north) + (\i*0.35 +1.18, +0.4cm)$) (token-\i) {\token};
%			\draw[-stealth] ([xshift=0cm]token-\i.south |- ChemFM-MG.north) -- (token-\i.south);
%		}
%		\node[draw=myred, rectangle, fill=color_activate_token, right=of token-6, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-7) {\textcolor{myred}{\textsc{EOS}}};
%		\draw[-stealth]([xshift=0cm]token-7.south |- ChemFM-MG.north) -- (token-7.south);
\end{scope}

==> figures/property_prediction.tex <==
%% property prediction

\begin{scope}[shift={(0.05,4)}]
	\node[draw=none, fill=color_property_prediction_bg, rounded corners=6.0, minimum width=7.6cm, minimum height=3.6cm, opacity=0.3, anchor=north west] (property_prediction) at (0, 4) {};
	\node[anchor=north west] at (property_prediction.north west) {\small \bfseries a\,    \small \ttfamily \bfseries Property Prediction};
	
	\node[draw, fill=color_chemFM, text centered, rounded corners, minimum width=7cm, minimum height=0.8cm, align=center] (ChemFM-PP) at (3.8, 1.5) {\footnotesize ChemFM};
	
	
	\foreach \token [count=\i] in {C,C,C,1,$($,C,C,$($, $=$, O, $)$, N, C, 1, $=$, O, $)$, C} {
		\node[rectangle, draw, fill=none,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-PP.south) + (\i*0.35 -3.6, -0.4cm)$) (token-\i) {\token};
		\draw[-stealth] (token-\i.north) -- ([xshift=0cm]token-\i.north |- ChemFM-PP.south);
	}
	\node[draw=myred, rectangle, fill=none, right=of token-18, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-19) {\textcolor{myred}{\textsc{EOS}}};
	\draw[-stealth] (token-19.north) -- ([xshift=0cm]token-19.north |- ChemFM-PP.south);
	
	\node[rectangle, draw, fill=Cyan!20, minimum height=0.4cm, minimum width=0.8cm, inner sep=1pt, outer sep=0pt, font={\tiny}, rounded corners=2.0] (mlp) at ($(token-19.north) + (0, 1.5)$) {MLP};
	\draw[-stealth] ([xshift=0cm]mlp.south |- ChemFM-PP.north) -- (mlp.south);
	\draw[-stealth] ($(mlp.north)+(-0.2, 0.0) $ ) -- ($(mlp.north) + (-0.2, 0.25)$ ) node[midway, above, font=\footnotesize, yshift=0.5mm] {$0$};
	\draw[-stealth] ($(mlp.north)+(+0.2, 0.0) $ ) -- ($(mlp.north) + (+0.2, 0.25)$ ) node[midway, above, font=\footnotesize,
	yshift=0.5mm] {$1$};
	
	\node[anchor=base] (icon1) at (0.25, 2.80) {\includegraphics[height=1em]{./figures/main_fig_elements/think_emoji}};
	\node[anchor=base, right=-1mm of icon1, align=left, text width=6cm] (text) at (icon1.east) {\fontsize{6.5}{7.5}\selectfont
	\baselineskip=3pt
	Predicting side effects of hepatobiliary and gastrointestinal disorders for \par};
	\node[anchor=base, right=-20mm of text, yshift=2mm] (icon2) at (text.east) {\includegraphics[height=4.6em,page=1]{./figures/main_fig_elements/pp_smiles.pdf}};	
\end{scope}



==> figures/radar_plots_generations.tex <==
\begin{figure}	
	

%\tikzsetnextfilename{moleculenet_radar}
\subfloat{\input{figures/moleculenet_radar}}
\hspace{-2em}
%\tikzsetnextfilename{admet_radar_1}
\subfloat{\input{figures/admet_radar_1}}
\hspace{-2em}
%\tikzsetnextfilename{admet_radar_2}
\subfloat{\input{figures/admet_radar_2}}

\end{figure}



==> figures/reaction_prediction.tex <==
\begin{scope}[shift={(7.75,4)}]
	\node[draw=none, fill=color_reaction_bg, rounded corners=6.0, minimum width=8.2cm, minimum height=3.6cm, opacity=0.3, anchor=north west] (reaction) at (0, 4) {};
	\node[anchor=north west] at (reaction.north west) {\small \bfseries c\, \small \ttfamily \bfseries Reaction Prediction};
	
	
	\node[draw, fill=color_chemFM, text centered, rounded corners, minimum width=8.0cm, minimum height=0.8cm, align=center] (ChemFM-RP) at (4.1, 1.5) {\footnotesize ChemFM};
	\foreach \token [count=\i] in {C, C, $($, Br, $)$, C, Br, $.$, C, C, $($, C, $)$, $=$, O} {
			\node[rectangle, draw, fill=none,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-RP.south) + (\i*0.35 -4.2, -0.4cm)$) (token-\i) {\token};
			\draw[-stealth] (token-\i.north) -- ([xshift=0cm]token-\i.north |- ChemFM-RP.south);
		}
	\node[draw=myred, rectangle, fill=none, right=of token-15, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-16) {\textcolor{myred}{\textsc{EOS}}};
	\draw[-stealth] (token-16.north) -- ([xshift=0cm]token-16.north |- ChemFM-RP.south);
	
	\foreach \token [count=\i] in {C,C,1,C,O,1} {
		\node[rectangle, draw, fill=color_activate_token,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-RP.north) + (\i*0.35 +1.18, +0.4cm)$) (token-\i) {\token};
		\draw[-stealth] ([xshift=0cm]token-\i.south |- ChemFM-RP.north) -- (token-\i.south);
	}
	\node[draw=myred, rectangle, fill=color_activate_token, right=of token-6, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-7) {\textcolor{myred}{\textsc{EOS}}};
	\draw[-stealth]([xshift=0cm]token-7.south |- ChemFM-RP.north) -- (token-7.south);
	
	
	
	
	\node[anchor=base] (icon1) at (0.25, 2.80) {\includegraphics[height=1em]{./figures/main_fig_elements/think_emoji}};
	\node[anchor=base, right=-1mm of icon1, align=left, text width=6cm] (text) at (icon1.east) {\fontsize{6.5}{7.5}\selectfont
		\baselineskip=3pt
		Predicting products of the reaction for \par};
	\node[anchor=base, right=-15mm of icon1] (reactant_1) at (text.east) {\includegraphics[height=4.5em,page=1]{./figures/main_fig_elements/reactant_1.pdf}};
	\node[anchor=base, right=-3mm of reactant_1] (text) at (reactant_1.east) {$+$};
	\node[anchor=base, right=-3mm of text, yshift=0.5mm] (reactant_2) at (text.east) {\includegraphics[height=4.2em,page=1]{./figures/main_fig_elements/reactant_2.pdf}};
	
%	\node[anchor=base, right=-20mm of text, yshift=2mm] (icon2) at (text.east) {\includegraphics[height=4.6em,page=1]{./figures/main_fig_elements/pp_smiles.pdf}};	
\end{scope}



%		\node[anchor=north west] at (reaction.north west) {\small \ttfamily \bfseries Reaction Prediction};
%		\node[anchor=base] (icon1) at (9.6, 2.69) {\includegraphics[height=1em]{./figures/main_fig_elements/think_emoji}};
%		\node[anchor=base, right=-2mm of icon1] (reactant_1) at (icon1.east) {\includegraphics[height=3.6em,page=1]{./figures/main_fig_elements/reactant_1.pdf}};
%		\node[anchor=base, right=-3mm of reactant_1] (text) at (reactant_1.east) {$+$};
%		\node[anchor=base, right=-3mm of text] (reactant_2) at (text.east) {\includegraphics[height=3.6em,page=1]{./figures/main_fig_elements/reactant_2.pdf}};
%		\node[anchor=base, right=-3mm of reactant_2] (text_1) at (reactant_2.east) {$=$ ?};
%		
%		%	\draw [rounded corners = 6.0, draw=none, fill=color_reaction_bg, opacity=0.3] (9.3,0.55) rectangle (15.95,3.58);
%		%	\node[minimum width=2.5cm, minimum height=1cm, align=center] (reaction) at (11.0,3.3) {\small \ttfamily \bfseries Reaction Prediction};
%		
%		
%		\node[draw, fill=color_chemFM, text centered, rounded corners, minimum width=6.6cm, minimum height=0.5cm, align=center] (ChemFM-RP) at (12.65, 1.6) {\footnotesize ChemFM};
%		\foreach \token [count=\i] in {C, C, N, $($, C, C, $)$, C, C, $.$, C, C, O, $.$, Cl} {
	%			\node[rectangle, draw, fill=none,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-RP.south) + (\i*0.35 -3.5, -0.4cm)$) (token-\i) {\token};
	%			\draw[-stealth] (token-\i.north) -- ([xshift=0cm]token-\i.north |- ChemFM-RP.south);
	%		}
%		\node[draw=myred, rectangle, fill=none, right=of token-15, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-16) {\textcolor{myred}{\textsc{EOS}}};
%		\draw[-stealth] (token-16.north) -- ([xshift=0cm]token-16.north |- ChemFM-RP.south);
%		
%		\foreach \token [count=\i] in {O, Cl} {
	%			\node[rectangle, draw, fill=color_activate_token,  minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] at ($ (ChemFM-RP.north) + (\i*0.35 +1.88, +0.4cm)$) (token-\i) {\token};
	%			\draw[-stealth] ([xshift=0cm]token-\i.south |- ChemFM-RP.north) -- (token-\i.south);
	%		}
%		\node[draw=myred, rectangle, fill=color_activate_token, right=of token-2, xshift=-0.90cm, minimum height=0.3cm, minimum width=0.3cm, font={\tiny}, inner sep=1pt, outer sep=0pt] (token-3) {\textcolor{myred}{\textsc{EOS}}};
%		\draw[-stealth]([xshift=0cm]token-3.south |- ChemFM-RP.north) -- (token-3.south);

%\draw [rounded corners = 6.0, draw=none, fill=red!20] (9.3,0.55) rectangle (15.95,4.);

==> methods/experimental_setting_comparison_on_admet.tex <==
\subsection{Experimental setting for molecular property prediction on ADMET}

We also compare ChemFM with methods on the leaderboard of the ADMET benchmark\cite{admet},
which comprises $22$ datasets and provides standard data splits and performance evaluation metrics.
%
The leaderboard facilitates cross-method comparisons on these datasets. 
%
However, 
not all methods on the leaderboard are evaluated correctly.
For example, common reasons for mis-evaluation include optimizing hyperparameters using the test datasets and combining the training and validation datasets for model training (practices that can improve performance, especially in the ADMET benchmarks, where most datasets contain fewer than 1,000 instances).
%
We carefully review the public codes of the methods on the leaderboard and excluded those that are mis-evaluated. 
%
The methods and corresponding reasons for exclusion are listed in the Supplementary Information.

For each dataset, we first conduct a hyperparameter search for the ChemFM-3B model. 
%
The adapted ChemFM-3B model outperforms the best models on the leaderboard for 20 out of the 22 datasets, with the exceptions being the Caco2\_Wang and HIA\_Hou datasets. 
%
For these two datasets, we then perform a hyperparameter search for the ChemFM-1B model,
which can achieve state-of-the-art results. 
%
The comparison between ChemFM and the previous best models is presented in Extended Data Table~\ref{table:rst_prop_prediction_admet}, with the hyperparameters used detailed in Extended Data Table~\ref{}.

==> methods/experimental_setting_comparison_on_moleculenet.tex <==
\subsection{Experimental setting for molecular property prediction on MoleculeNet}

% moleculenet
We begin by fine-tuning the ChemFM model on datasets from the MoleculeNet benchmark\cite{moleculenet}. 
%
While many methods have been developed and evaluated on MoleculeNet benchmark, 
comparisons between them are often problematic due to variations in dataset splitting strategies
and random seed selections across studies.
%
This issue is particularly exacerbated with the ``scaffold'' split, which partitions molecules based on structural scaffolds.
%
Although this method creates more structurally diverse and challenging train/validation/test folds than random splitting,
it can result in significantly different test sets across experiments, complicating cross-study comparisons.

To ensure a comprehensive evaluation of ChemFM, we conduct three distinct sets of comparisons with existing methods, all using the exact same train/validation/test datasets. 
%
We exclude methods that are not open-sourced as verifying their dataset splits is not possible.

\noindent \textbf{Comparison set 1:}
We first fine-tune both ChemFM-1B and ChemFM-3B models on standard MoleculeNet datasets\cite{moleculenet,chembench}, as provided in the MoleculeNet paper. 
%
The methods we compare against include MoleculeNet models\cite{moleculenet}, Direct Message Passing Neural Networks (D-MPNN or Chemprop)\cite{dmpnn}, and MolMapNet (MMNB)\cite{MMNB}.
%
We conduct a random search for the hyperparameters and LoRA configurations for each dataset, with the selected hyperparameters detailed in Extended Data Table~\ref{}.
%
Importantly, 
hyperparameter tuning is based solely on validation performance, 
and no tuning is performed on the test datasets.
%
We evaluate our models across three folds and report the average performance, along with the corresponding split method and evaluation metrics, in Extended Data Table~\ref{table:rst_prop_prediction}.

\noindent \textbf{Comparison set 2:}
We then compare ChemFM with the AttentiveFP method\cite{attentiveFP}, 
which uses random splits with different seeds than the standard MoleculeNet benchmark. 
%
MMNB provides a direct comparison with AttentiveFP (as shown in Table 2 of the MMNB paper\cite{MMNB}), 
where MMNB outperforms AttentiveFP on most datasets. 
%
Since our ChemFM models consistently outperform MMNB, we reasonably infer that ChemFM is also superior to AttentiveFP on these datasets. 
%
However, in four specific datasets---Tox21, ESOL, FreeSolv, and Lipophilicity---AttentiveFP outperforms MMNB. 
%
For these datasets, we conduct a direct comparison by reevaluating AttentiveFP across three folds with different random seeds and fine-tuning ChemFM using identical data splits. 
%
The results are presented in Extended Data Table~\ref{table:rst_prop_prediction_attentive_fp}.

\noindent \textbf{Comparison set 3:}
The third comparison set focuses on methods using a deterministic scaffold split to generate a single fold of train/validation/test sets, including 3D InfoMax\cite{3dinfomax}, Mole-BERT\cite{molebert}, GraphMVP\cite{graphmvp}, and MoleculeSDE\cite{moleculeSDE}. 
%
We adopt the same settings as these methods---training on the same data fold with three different random seeds (this seed only affect the training procedure like the network weights initialization network dropout, will not affect the dataset splitting)---and report the average performance in Extended Data Table~\ref{table:rst_prop_prediction_molebert}.


It is important to highlight that no additional hyperparameter tuning is performed for comparison sets 2 and 3. 
We reuse the hyperparameters optimized for the standard MoleculeNet datasets (shown in Extended Data Table~\ref{}), despite differences in splitting methods and random seeds. 
%
For each dataset, we first fine-tune the ChemFM-3B model, as it outperforms ChemFM-1B in the standard MoleculeNet benchmarks. 
%
If ChemFM-3B does not outperform all other methods (specifically, the ESOL dataset in comparison set 2 and the MUV dataset in comparison set 3), we proceed to fine-tune ChemFM-1B.
%
The results indicate that at least one of our ChemFM models outperform all other compared methods across the evaluated datasets, even without additional hyperparameter tuning on these specific data folds.

==> methods/experimental_setting_on_uspto.tex <==
\subsection{Experimental setting for reaction prediction on USPTO}

==> methods/finetune.tex <==
\subsection{Datasets for fine-tuning}\label{sec:finetune_dataset
}
To enable our model as a versatile tool applicable across diverse chemical contexts, we have curated a comprehensive collection of $32$ commonly-used datasets, crafting $\textcolor{red}{500,000}$ text instances across $11$ distinct subtasks.
%
These subtasks can be summarized into three broad categories of tasks: molecular property prediction, molecule generation, and chemical reaction-related tasks.

Given the varied sizes of these datasets, ranging from as extensive as \textcolor{red}{100,000} entries to as concise as \textcolor{red}{10,000} entries, ensuring equitable learning across all is paramount. 
%
Thus, we employ augmentation and interleaving techniques, amalgamating the datasets into a unified corpus of $\textcolor{red}{1,000,000}$ instances.
%
Further details regarding the constituent datasets and the methodology employed for their integration are outlined in Extended Table \ref{}.





\subsection{Training details for fine-tuning }\label{sec:finetune_train}

\begin{enumerate}
	\item Properties prediction: \\
	\cbos{MolStr}\eos\resulting\pbos{PropStr}\eos
	\item Molecule prediction conditioned on properties: \\
	\pbos{PropStr}\eos
\resulting\cbos{MolStr}\eos
	\item Molecule reconstruction conditioned on properties and masked molecule:\\
	\pbos{PropStr}\eos\mcbos{MaskedMolStr}\eos\resulting\cbos{MolStr}
\eos
	\item Molecule prediction conditioned on scafold:\\
	\sbos{ScafoldStr}\eos\resulting\cbos{MolStr}\eos
	\item Molecule prediction conditioned on scafold and properties: \\
	\pbos{PropStr}\eos\sbos{ScafoldStr}\eos\resulting\cbos{MolStr}\eos
	\item Products prediction conditioned on reactants: \\
	\rctbos{RctStr}\eos\resulting{ProdStr}\eos
	\item Reaction property prediction conditioned on reactants and products of the reaction: \\
	\rctbos{RctStr}\eos\prodbos{ProdStr}\eos\resulting\pbos{PropStr}\eos
	\item Missing reactant prediction conditioned on products: \\
	\mrctbos{MaskedRctStr}\eos\prodbos{ProdStr}\eos\resulting\cbos{MolStr}\eos
	\item Missing reactant prediction conditioned on products and properties: \\
	\pbos{PropStr}\eos\mrctbos{MaskedRctStr}\eos\prodbos{ProdStr}\eos\resulting\cbos{MolStr}\eos
	\item Reactants prediction conditioned on products and properties:\\
	\pbos{PropStr}\eos\prodbos{ProdStr}\eos\resulting\rctbos{RctStr}\eos
	\item Reactants prediction conditioned on products: \\
	\prodbos{ProdStr}\eos\resulting\rctbos{RctStr}\eos
\end{enumerate}

==> methods/finetune_dataset.tex <==
\subsection{Fine-tuning datasets}\label{sec:finetune_dataset}
We collect a comprehensive dataset consisting of  $30$ widely-used datasets across diverse chemical application scenarios, totaling $50000$\todo{check the size} entries.
%
The final fine-tuning dataset is obtained through a series of preprocessings. 

First, a single entry can be applied to multiple tasks by phrasing it based on task-specific templates.
%
For example, entries containing pairs of molecules and their properties can serve for both  property prediction and molecule conditioning generation tasks.
%
Similarly, entries comprising complete reaction chains are suitable for both forward synthesis and retro-synthesis prediction tasks.

Given the considerable variance in dataset sizes, ranging from $1000$ entries to $100000$ \todo{check the number} entries,
a naive concatenation of the datasets could lead the training to a bias towards satisfication of larger-datasets, potentially neglecting smaller ones.
%
We employ the data augmentation technique for datasets but the augmentation scales are based on the their size, wherein smaller datasets undergo multiple folds of augmentation compared to larger ones.
%
SMILES enumeration \cite{smilesaug} is used for molecule augmentation, while root-aligned SMILES (R-SMILES) \cite{rsmiles} is for reaction augmentation.
%
The augmentation not only enhance data utilization efficiency but also improve the model performance in property and reaction prediction tasks \cite{property_prediction_with_aug,rsmiles}.

Furthermore, the imbalances inherent in the dataset sizes can be further mitigated by employing an interleaving strategy during dataset construction. 
%
This strategy mixes datasets by alternately selecting examples from each dataset, effectively oversampling small-sized datasets with a higher sampling probability compared to larger datasets.
 
The resulting fine-tuning dataset comprises a total of $50000$\todo{check the size} text instances. 
%
Further  details regarding the dataset construction is presented in Extended Figure \ref{}.


==> methods/finetune_detail.tex <==
\subsection{Fine-tuning details}\label{sec:finetune_train}

We employ the full-parameter fine-tuning for two pre-trained variants, AIChemy-1B and AIChemy-3B, on the comprehensive downstream dataset.
%
The fine-tuning objective remains consistent with the pre-training phase: predicting the next token in a sequence based on the context of previous tokens.
%
During the pre-training, the cross-entropy loss is evaluated on each token, with all losses contributing to the final loss for model optimization.
%
However, during the fine-tuning, only the loss on the output tokens---those subsequent to the \resulting token---contributes to the final loss. 
%
This fine-tuning strategy is similar to the approach used for fine-tuning in the question-answering chatbot \cite{tinyllama}.

For the fine-tuning process, we utilize an AdamW optimizer with a fixed learning rate of $1 \times 10^{-5}$. The fine-tuning is performed on a single NVIDIA HGX H100 node. 
%
The models are trained for $5$ epochs, with fine-tuning durations of $128$ and $256$ hours for AIChemy-1B and AIChemy-3B, respectively.

==> methods/finetune_template.tex <==
\subsection{Task templates}\label{sec:finetune_template}
To enable the handling of diverse chemical tasks, we employ different templates to standardize these tasks within a unified language generation framework:
\begin{enumerate}
	\item Properties prediction: \\
	\cbos{MolStr}\eos\resulting\pbos{PropStr}\eos
	\item Molecule generation conditioned on properties: \\
	\pbos{PropStr}\eos\resulting\cbos{MolStr}\eos
%	\item Molecule reconstruction conditioned on properties and masked molecule:\\
%	\pbos{PropStr}\eos\mcbos{MaskedMolStr}\eos\resulting\cbos{MolStr}\eos
	\item Molecule prediction conditioned on scaffold:\\
	\sbos{ScaffoldStr}\eos\resulting\cbos{MolStr}\eos
	\item Molecule prediction conditioned on scaffold and properties: \\
	\pbos{PropStr}\eos\sbos{ScaffoldStr}\eos\resulting\cbos{MolStr}\eos
	\item Products prediction conditioned on reactants: \\
	\rctbos{RctStr}\eos\resulting{ProdStr}\eos
	\item Reaction property prediction conditioned on reactants and products of the reaction: \\
	\rctbos{RctStr}\eos\prodbos{ProdStr}\eos\resulting\pbos{PropStr}\eos
%	\item Missing reactant prediction conditioned on products: \\
%	\mrctbos{MaskedRctStr}\eos\prodbos{ProdStr}\eos\resulting\cbos{MolStr}\eos
%	\item Missing reactant prediction conditioned on products and properties: \\
%	\pbos{PropStr}\eos\mrctbos{MaskedRctStr}\eos\prodbos{ProdStr}\eos\resulting\cbos{MolStr}\eos
%	\item Reactants prediction conditioned on products and properties:\\
%	\pbos{PropStr}\eos\prodbos{ProdStr}\eos\resulting\rctbos{RctStr}\eos
	\item Reactants prediction conditioned on products: \\
	\prodbos{ProdStr}\eos\resulting\rctbos{RctStr}\eos
\end{enumerate}

In these templates, ``MolStr'', ``ScaffoldStr'', ``RctStr'', and ``ProdStr'' denote molecule, scaffold, reactant, and product strings, respectively, represented by SMILES. 
%
It is important to note that a reactant or product might consist of multiple molecules participating in the reaction, separated by ``.''.
%
The ``PropStr'' denotes a property string, as introduced in Sec. \ref{sec:numerical_representation}, representing properties of a molecule or reaction.
%
Special tokens such as \cbos, \sbos, \pbos, \rctbos, and \prodbos are utilized to signify the beginnings of molecule, scaffold, property, reactant, and product strings respectively, with each string concluding with an \eos token.
%
The token \resulting is utilized to separate the input prompt from output response, indicating the conditions for the task preceding it and the results following it.

==> methods/numerical_embedding.tex <==
\subsection{Property representation} \label{sec:numerical_representation}
\todo{this section is also too detail, maybe we can move to other part in the paper.}
The property string consists of single or multiple property substrings, 
each containing the property name alongside its corresponding value.
%
The property name serves as a unique identifier for each specific property of a molecule or reaction and is represented by a special token $\langle \text{PropName} \rangle$.
%
The property value can take two forms: discrete classification labels or continuous regression values. 
%
It is important that the representation of these values should be compatible with both property conditioning and prediction scenarios.

For classification tasks, which align with the objectives of causal language modeling---predicting probability distributions over different vocabularies or categories---tokenizing label indexes into distinct class tokens seamlessly incorporate the classification task into the framework of causal language modeling. 
%
Hence, a class label index $i$, for instance, is tokenized as $\langle \text{c}i \rangle$.

% regression
Regarding regression, embedding continuous real values presents challenges.
%
Conventional methods typically require an additional MLP layer to either encode the values into or extract them from embeddings \cite{ccgan,bert}, but such a technique complicates the architecture and alters the training objective. 
%
Alternatively, treating digits of values as distinct characters allows for individual embedding and tokenization.  
%
Similar to positional encodings, numerical encodings can be added to the embeddings to convey numerical semantic proximity to digit tokens \cite{regressiontrasformer}.

However, comprehensive ablation studies (Sec. \ref{?} of the Supplementary Information) indicate that introducing numerical encodings does not improve the performance of property prediction or conditioning scenarios. 
%
This is attributed to the language model's ability to learn numerical orderings from the extensive corpus data, as validated in Sec. \ref{?} of the Supplementary Information.

%
In this work, the real numbers are represented by breaking them down into individual digits and their corresponding decimal places.
%
To formalize this, let's consider a non-negative real value $r$.
%
We represent $r$ as $n$ tokens $ \langle v_1\_p_1 \rangle \ldots \langle v_i \_ p_i \rangle  \ldots \langle v_n\_p_n \rangle $ from highest decimal position $p_1$ to lowest $p_n$, 
where $v_i$ represents a digit ($0$ to $9$). 
%
Thus, the real value $r$ can be expressed as $\sum_{i=1}^{n} v_i^{p_i}$.
%
Additionally, to represent negative values, we prepend a special token $\langle - \rangle$ to the sequence. 

%
For instance, two properties---one named $\text{P}1$ with a classification label index $3$ and the other named $\text{P}2$ with a regression value $-3.12$—can be represented as:
\begin{equation*}
	\langle \text{P1} \rangle \langle : \rangle \langle \text{c}3 \rangle 
	\langle ; \rangle
	\langle  \text{P2} \rangle \langle : \rangle \langle - \rangle \langle 2\_0 \rangle \langle 5\_-1 \rangle \langle 3\_-2 \rangle \langle 3\_-2 \rangle.
\end{equation*} 
Here, the special token $\langle : \rangle$ separates the property name and property value, while $\langle ; \rangle$ separates different properties. 


%For instance, $-12.533$ would be represented as $\langle - \rangle \langle 1\_1 \rangle \langle 2\_0 \rangle \langle 5\_-1 \rangle \langle 3\_-2 \rangle \langle 3\_-2 \rangle$. 


%A non-negative real value $r$ can be represented as a series of tokens $\langle v_i\text{\_}p_i \rangle$, where $v_i\in[0\ldots9]$ represents the digit value and $p_i \in $ denotes the decimal place. so that $r = \sum_{i=p_\text{min}}^{p_\text{max}} v_i^{p_i}.$
%
%
%Continuous real numbers $r$ are converted into 
%
%
% containing its digit and decimal place. 
%%
%For example, $12.533$ will be segmented into $\{ \}$ 
%
%
% are treated as plain text and divided into distinct numbers for representation and tokenization in this work.
%%
%For instance, 


\todo{for both classification and regression, give an example}

==> methods/parameter_efficient_finetuing.tex <==
\subsection{Parameter-efficient fine-tuning}

==> methods/pretrain.tex <==
\subsection{Details for pre-training}\label{sec:pretrain}

% Molecule representation and tokenization
Molecules are normally encoded as serialization formats or graph structures to enable the use of established sequence-based or graph-based networks to tackle complex chemical tasks. 
%
ChemFM is a sequence-based model, and specifically, by employing the simplified molecular input line entry system (SMILES), a widely-used molecular serialization formats in computational chemistry\cite{attentiveFP,molgpt,root_smiles}, 
molecules are transformed into SMILES strings 



Deep learning models that are used for chemical tasks often rely on molecular representations encoded as serialization formats or graph structures


ChemFM is a sequence-based model that consumes the serialization formats of the molecules structure


relies on molecular representations encoded in serialization formats.


The pre-training of the ChemFM aims to learn the general chemical knowledge 

ChemFM follows the training paradigm of the modern LLM

%% SELFIES: PANGU/MITPretrain/RegressionTransformer/CLM
ChemFM is a sequence-based model that relies on molecular representations encoded in serialization formats.
%
Specifically, we employ the simplified molecular input line entry system (SMILES), a widely-used molecular serialization formats in computational chemistry\cite{attentiveFP,molgpt,root_smiles}.
%
Molecules are first transformed into SMILES strings using the RDKit library\cite{rdkit}. 
%
These SMILES strings are then segmented and tokenized using subword tokenizer\cite{bpe} with $266$ predetermined vocabularies. 
%
The vocabulary includes both uppercase and lowercase representations of the $118$ elements from the periodic table, numerical digits from $0$ to $9$, $19$ special symbols as specified by SMILES syntax \cite{smiles}, and a special end token indicating the termination of a SMILES string. 

These tokens form the foundational vocabulary used during the pre-training phase, while additional special tokens are introduced during fine-tuning to address specific task requirements.


%The pre-training dataset exclusively contains molecules represented by SMILES and does not involve any downstream tasks.
%%
%It aims to learn the syntax and semantic rules of the SMILES system and learn molecular fingerprints or the features to embed them in the latent space representation of the model.
%
%We adopt a mixture of approximately 1.1 trillion molecules from ZINC20\cite{zinc} ($90\%$) and PubChem \cite{pubchem} ($10\%$) as the pre-trained large-scale dataset. 
%%
%During the pre-training, we balance sampling from both datasets until ZINC20 data are exhaustively trained for one epoch, providing roughly $9$ epochs of training for PubChem dataset.
%%
%In total, the pre-training consumes around $\textcolor{red}{950}$ trillion tokens. 
%
%Our trainings are run on two NVIDIA DGX H100 nodes, each equipped with $8x$H100 GPUs.
%%
%The training duration amounted to $\textcolor{red}{128}$ hours for the 1B model and $\textcolor{red}{256}$ hours for the 3B model. 
%%
%For further details on our training setup, please refer to Extended Table \ref{} for a comprehensive summary of the parameters used.



==> methods/tokenization.tex <==
\subsection{Text representations and tokenizations}\label{sec:tokenization}

The input text strings for the chemical model comprises three components: 
%
1) special tokens denoting the types and pipelines of the chemical tasks,
%
2) strings representing the molecular structures,
%
and 3) numerical values indicating either the properties of the molecules or the reactions.
%
In this section, we detail the representations and tokenizations of both the molecules and numerical values. 
%
Special tokens will be introduced in Sec.~\ref{sec:finetune_train}, which discusses string template construction for different downstream tasks. 

\subsubsection{Molecule representation}

%% SELFIES: PANGU/MITPretrain/RegressionTransformer/CLM

SMILES \cite{smiles} system enables the representation of molecular structures through a linear string of symbols.
%
It was invented in $1988$ and has been widely used in computational chemistry \cite{attentiveFP,molgpt,root_smiles}. 
%
However, the SMILES system suffers from a significant drawback: despite adherence to its grammatical rules, the resulting SMILES string may yield an invalid molecular representation \cite{selfies}, potentially deviating from a molecular graph or violating chemical rules.  

The introduction of SELFIES \cite{selfies} aims to address this limitation by guaranteeing a $100\%$ robust and valid molecular string representation when composed according to its grammatical rules. 
%
Such robustness holds crucial importance for generative models in molecular research, leading to a growing trend in favor of SELFIES as a replacement for SMILES \cite{pangu, regressiontrasformer, mit_pretrain}.

Nevertheless, contemporary LLMs are typically extensively trained, and thus, semantic rules should not pose a significant challenge to sufficiently trained models. 
%
Analogous to natural language models, which do not initially encode grammar and semantic information, LLMs can acquire grammatical understanding over time and generate sentences with minimal grammatical errors after sufficient training.
\todo{Feiyang: the SMILES and SELFIES introductions may be too detailed and we can move them to introduction or results.}


Therefore, it is imperative to reevaluate the advantages offered by SELFIES also benefit large chemical models.
%
To this end, we conduct a comprehensive set of comparative experiments involving SMILES and SELFIES across property prediction and molecule generation tasks (see Sec.~\ref{sec:ablation_study_molecule_string} in Supplementary Information). 
%
Our studies reveal minimal disparity between the two molecular representations concerning the property prediction task.  
% 
However, in the molecule generation task, we observe that the model using SMILES can generate nearly $100\%$ valid molecules. 
%
Additionally, compared to the SELFIES-based model, the SMILES-based model outperforms in property-conditional molecule generation task and can generate molecules that better align with conditioned attributes.

We hypothesize and subsequently conduct experiments to validate that this discrepancy arises from the instability of SELFIES representations. 
%
Even minor alterations to SELFIES symbols can result in significant changes in molecular structure (\textcolor{red}{see Sec. ? in Supplementary Information}), thus adversely affecting the properties of molecules. 
%
Consequently, the SMILES system proves to be a better fit for large chemical models and is adopted as the molecule representation method in our work.


The SMILES strings are split and tokenized into a total of $192$ \todo{please check} tokens, including uppercased and lowercased $118$ elements from the periodic table, numerical digits from 0 to 9, and 20 special symbols as per SMILES syntactic specifications \cite{smiles}. 
%
The vocabularies (\textcolor{red}{tokens?}) used for representing molecules are summarized in \textcolor{red}{Extended Table \ref{}}.



\subsubsection{Numerical embedding}

A property string comprises both the property name and its corresponding value. 
%
The property name serves as a unique identifier for each distinct property, as detailed in Sec.~\ref{sec:finetune_train}. 
%
Embedding property values into the language model is essential to both property embedding and prediction scenarios. 
%
These values can manifest in two forms: discrete classification labels or continuous regression values.

Assigning distinct class labels to different class tokens embeds category information into the language model, and can also be used for class prediction, because such a task aligns to the cross-entropy loss in the causal language modeling.
%
However, embedding continuous real regression labels presents challenges.
%
Conventional methods involve introducing an additional MLP layer to encode or extract the values from embedding layers, potentially complicating the architecture and altering the training objective. 
%
Alternatively, treating digits of values as distinct characters allows for individual embedding and tokenization.  
%
Similar to positional encodings, numerical encodings can be added to the embeddings to convey numerical semantic proximity to digit tokens \cite{regressiontrasformer}.

However, comprehensive ablation studies suggest that introducing numerical encodings does not improve the performance of property prediction or condition scenarios. 
%
This is attributed to the language model's ability to learn numerical orderings from the extensive corpus data, as validated in Sec. \ref{?} of the Supplementary Information.
%
Therefore, continuous real numbers are treated as plain text and divided into distinct numbers for representation and tokenization in this work.
\todo{for both classification and regression, give an example}




==> results/pretrain.tex <==
\subsection{Pre-training performance}
%
We pre-train both ChemFM variants (ChemFM-1B and ChemFM-3B) on the augmented UniChem\cite{unichem} dataset for slightly more than $1$ epoch.
%
he validation loss for both models steadily decreased throughout training, showing no signs of saturation even after processing $818$ billion tokens (Fig.?).
%
As expected, the final validation loss for ChemFM-3B is lower than that of ChemFM-1B. 
%
However, the final validation losses of both models slightly deviate from the predicted scaling law, suggesting that under the current data regime, further model scaling may lead to diminishing returns as the loss approaches a plateau (Methods and Extended Data Fig.~\ref{fig:scaling_law}). %\todo{do we need to have this scaling law analysis here? or we just have this part in the methods}
%of the ChemFM models on the augmented UniChem\cite{unichem} dataset for slightly more than $1$ epoch. 
%%
%The validation loss for both models continuously decreasing during the training, and there is no sign of saturation after pre-training on $818$ billion tokens.
%%
%No surprisingly, the final validation loss for ChemFM-3B is less than the one for ChemFM-1B model.
%%
%Yet, the final validation loss for ChemFM-1B and ChemFM-3B slightly deviate from the scaling law, 
%indicating that within the current data invariant, further scaling up the model could enter the loss plateaus and the
%return could be diminishing (Methods and Extended Data Fig.~\ref{fig:scaling_law}).  

We evaluate both ChemFM variants on non-conditional molecular generation, generating $\num{100000}$ molecules for each model (Table ?). %TODO: fixme
%
The results demonstrate that both models achieve high validity without additional constraints during tokenization, model training, or generation. 
%
ChemFM-3B achieves a marginally higher validity of $0.996$ compared to ChemFM-1B. 
%
These findings indicate that the models 
effectively capture the syntactic rules of SMILES, explicit chemical constraints, and the sequential dependencies inherent in molecular structures.
%
Both models also achieve a perfect uniqueness score of $1.0$, meaning all generated SMILES are distinct from one another.
% 
Furthermore, the models exhibit high internal diversity, indicating that the structures of the generated molecules are varied and diverse. 
%
By comparing various physicochemical descriptors---such as molecular complexity, weight, and structural characteristics---between the training set and the generated molecules, we observe that ChemFM faithfully captures the distribution of molecules in the training data without overfitting to a narrow subset.
%
More importantly, over half of the generated molecules are entirely novel, not found in the extensive training dataset, highlighting the potential of these models for exploring chemical space, discovering new molecules, and optimizing molecular structures.

%
%
%We benchmark both variants on non-conditional molecular generation, 
%randomly generating $\num{100000}$ molecules for each model (Table 1). 
%%
%The results demonstrate that both models achieve high validity without additional constraints introduced during tokenization, model training, or generation.
%%
%ChemFM-3B achieves a marginally higher validity of $0.996$ compared to ChemFM-1B.
%%
%These results indicates that the models effectively capture the syntactic rules of SMILES, explicit chemical constraints, and the sequential dependencies inherent in molecular structures.
%
%Furthermore, both models exhibit high uniqueness and internal diversity scores
%
%achieve high unique scores and internal diversity, meaning that the vast majority of generated molecules are distinct. 
%%
%By comparing a variety of physicochemical descriptors---such as complexity, molecular weight, and structural information---between the training set and the generated molecules, we find that ChemFM effectively captures the distribution of molecules in the training set without collapsing into a narrow region of the dataset.
%
%More importantly, over half of the generated molecules are entirely novel, not present in the enormous amount training database, showcasing the potential of our models in exploring chemical space, including discovering new molecules and optimizing molecular structures.


 

==> results/property_prediction__copy_.tex <==

\subsection{Molecular property prediction}
We fine-tune AIChemy-1B and AIChemy-3B on a comprehensive molecular property prediction dataset 
comprising $20$ \todo{check the number} datasets, which include $50$ classification and $10$ regression properties.
%
We showcase the fine-tuned models' performance across $10$ standard  benchmarks, involving $20$ \todo{check the number} classification and $5$ regression properties (refer to Table~\ref{table:rst_prop_prediction}).

\subsection{Molecule property prediction}
We evaluate the adaption ability of ChemFM molecular property prediction on two widely-used molecular property prediction benchmarks:
(1) MoleculeNet\cite{wu2018moleculenet} and
(2) Admet\cite{huang2021therapeutics}.
%


a comprehensive molecular property prediction dataset 
comprising $20$ \todo{check the number} datasets, which include $50$ classification and $10$ regression properties.
%
We showcase the fine-tuned models' performance across $10$ standard  benchmarks, involving $20$ \todo{check the number} classification and $5$ regression properties (refer to Table~\ref{table:rst_prop_prediction}).
%
As illustrated in the table, AIChemy demonstrates superior performance compared to other state-of-the-art models that are trained individually for each datasets. 
%
For example, in classification tasks, AIChemy exhibits a minimum improvement of $0.1$ in the area under the receiver operating curve (ROC-AUC) metric on the BBBP dataset, and a remarkable maximum improvement of $3.0$ on the BACE dataset.
%
In regression tasks, AIChemy significantly reduces the root mean squared errors (RMSE), achieving improvements 
of $0.02$ on the ESOL dataset, $0.42$ on FreeSolv, $0.63$ on Lipophilicity, and $0.82$ on PDBbind dataset.
%
AIChemy also shows remarkable performance in predicting molecular properties other than standard benchmarks, and these results are provided in Extended Table \ref{}.
%
Our comprehensive analysis indicates that AIChemy excels in predicting a wider array of molecular properties in a single model.




We fine-tune ChemFM-1B and ChemFM-3B on a unified molecule property prediction dataset, 
encompassing $20$ \todo{check the number} datasets including $40$ classification and regression properties.
%
As 


classification and regression properties


We showcase the fine-tuned model's performance across $10$ standard  molecule property prediction benchmarks, encompassing $20$ \todo{check the number} classification and regression properties (refer to Table~\ref{table:rst_prop_prediction}).
%
As illustrated in the table, AIChemy demonstrates superior performance compared to other state-of-the-art models that are trained individually for each datasets. 
%
For example, in classification tasks, AIChemy exhibits a minimum improvement of $0.1$ in the area under the receiver operating curve (ROC-AUC) metric on the BBBP dataset, and a remarkable maximum improvement of $3.0$ on the BACE dataset.
%
In regression tasks, AIChemy significantly reduces the root mean squared errors (RMSE), achieving improvements 
of $0.02$ on the ESOL dataset, $0.42$ on FreeSolv, $0.63$ on Lipophilicity, and $0.82$ on PDBbind dataset.
%
AIChemy also shows remarkable performance in predicting molecular properties other than standard benchmarks, and these results are provided in Extended Table \ref{}.
%
Our comprehensive analysis indicates that AIChemy excels in predicting a wider array of molecular properties in a single model.

\input{tables/results_PropPred}

==> supplementary_infomation/ablation_studies.tex <==
%\subsection{Ablation Studies}
\renewcommand{\thesubsection}{\arabic{subsection}}

\subsection{Ablation studies with different string representations and tokenizations}
\subsubsection{Molecule string representations}
\label{sec:ablation_study_molecule_string}
\subsubsection{Numerical representations and tokenizations}
\label{sec:ablation_study_numerical_value}

\input{tables/ablation_study_prop_pred}
\input{tables/ablation_study_generation}


==> tables/ablation_study_generation.tex <==
\begin{table}[h]
	\caption{\textbf{Performance comparison in generation task using different string representations and tokenizations.}}
	\begin{tabular}{cccccc}
		
		\hline
		Molecule Encoding + Numerical Encoding & Validity $\uparrow$ & Uniqueness $\uparrow$ & Novelty $\uparrow$ & MAD $\downarrow$ & SD $\downarrow$\\
		%\hline
		%MolGPT & 0.972 & 0.998 & 0.967 & 0.054 & 0.050 \\ % this evaluation is rerun the molgpt code
		\hline
		%SMILES (less tokens) + Numerical Mapping  & 0.949 & 0.998 & 0.977 & 0.068 & 0.058 \\ % this smiles tokenizer is from the molgpt
		%SMILES (less tokens) + Numerical Mapping + Type Embedding  & 0.948 & 0.999 & 0.980 & 0.070 & 0.059 \\ % this smiles tokenizer is from the molgpt
		SMILES + Text Encoding & 0.959 & 0.999 & 0.975 & 0.060 & 0.054 \\ 
		SMILES + Numerical Mapping  & 0.951 & 0.999 & 0.978 & 0.066 & 0.059 \\
		%SELFIES + Numerical Mapping & 1.000 & 1.000 & 0.989 & 0.105 & 0.088 \\
		SMILES + Numerical Encoding & 0.949 & 0.999 & 0.979 & 0.063 & 0.056 \\
		SELFIES + Text Encoding & 1.000 & 1.000 & 0.985 & 0.094 & 0.080 \\
		\hline
	\end{tabular}
	\footnotetext{Mean average deviation (MAD), standard deviation (SD), validity, uniqueness, and novelty values for different encoding approaches in generation task; we use the single property ``QED" in GuacaMol dataset as an example.}
\end{table}

==> tables/ablation_study_prop_pred.tex <==
\begin{table}[h]
	\caption{\textbf{Performance comparison in property prediction task using different string representations and tokenizations.} \textcolor{red}{Just a placeholder}}
	\begin{tabular}{cccccc}
		
		\hline
		Molecule Encoding + Numerical Encoding & Validity $\uparrow$ & Uniqueness $\uparrow$ & Novelty $\uparrow$ & MAD $\downarrow$ & SD $\downarrow$\\
		%\hline
		%MolGPT & 0.972 & 0.998 & 0.967 & 0.054 & 0.050 \\ % this evaluation is rerun the molgpt code
		\hline
		%SMILES (less tokens) + Numerical Mapping  & 0.949 & 0.998 & 0.977 & 0.068 & 0.058 \\ % this smiles tokenizer is from the molgpt
		%SMILES (less tokens) + Numerical Mapping + Type Embedding  & 0.948 & 0.999 & 0.980 & 0.070 & 0.059 \\ % this smiles tokenizer is from the molgpt
		SMILES + Text Encoding & 0.959 & 0.999 & 0.975 & 0.060 & 0.054 \\ 
		SMILES + Numerical Mapping  & 0.951 & 0.999 & 0.978 & 0.066 & 0.059 \\
		%SELFIES + Numerical Mapping & 1.000 & 1.000 & 0.989 & 0.105 & 0.088 \\
		SMILES + Numerical Encoding & 0.949 & 0.999 & 0.979 & 0.063 & 0.056 \\
		SELFIES + Text Encoding & 1.000 & 1.000 & 0.985 & 0.094 & 0.080 \\
		\hline
	\end{tabular}
	\footnotetext{Mean average deviation (MAD), standard deviation (SD), validity, uniqueness, and novelty values for different encoding approaches in generation task; we use the single property ``QED" in GuacaMol dataset as an example.}
\end{table}

==> tables/finetune_dataset.tex <==
\begin{table}[h]
	\caption{\textbf{Fine-tuning datasets composition and construction.}} 	\label{table:fine-tune_dataset}
	\begin{tabular}{cccc}
		\toprule
	    \multirow{30}{*}{Interleave} &  &                                                         & moses2    \\
	    \cmidrule{2-4}
	                                 &  &                                                         & guacamol2 \\
	    \cmidrule{2-4}
	                                 &\multirow{3}{*}{Interleave} &  \multirow{2}{*}{Concatenate} & uspto\_mit  \\
	                                 &                            &                               & uspto\_50k  \\
	                                 \cmidrule{3-4}
	                                 &                            &                               & uspto\_full \\
	    \cmidrule{2-4}
	                                 &                            &                               & BACE        \\
	                                 &                            &                               & BBBP        \\
	                                 &                            &                               & Clearance   \\
	                                 &                            &                               & Clintox     \\
	                                 &                            &                               & Delaney     \\
	                                 &                            &                               & FreeSolv    \\
	                                 &                            &                               & HIV         \\
	                                 &                            &                               & HOPV        \\
	                                 &                            &                               & HPPB        \\
	                                 &                            &                               & Lipo        \\
	                                 &                            &                               & MUV         \\
	                                 &                            &                               & NCI         \\
	                                 &                            &                               & PCBA        \\
	                                 &                            &                               & PDBBind        \\
	                                 &                            &                               & PPB        \\
	                                 &                            &                               & QM7        \\
	                                 &                            &                               & QM8        \\
	                                 &                            &                               & QM9        \\
	                                 &                            &                               & SAMPL        \\
	                                 &                            &                               & SIDER        \\
	                                 &                            &                               & THERMOSOL        \\
	                                 &                            &                               & TOX21        \\
	                                 &                            &                               & TOXCAST        \\
	                                 &                            &                               & SUZUKI Couplings        \\
	                                 &                            &                               & Buchwald Hartwig        \\
	                                                         
		\botrule
	\end{tabular}
	\footnotetext{Hello}
\end{table}


==> tables/model_architecture_scaling_law.tex <==
\begin{table}[h]
	\caption{\textbf{Architectures of the ChemFM models.}} 	\label{table:model_architecture}
	\begin{tabular}{lccccccc}
		\toprule
		\thead{Model} &
		\thead{$n_\text{params}$} & \thead{$n_\text{layers}$} & \thead{$n_\text{heads}$} & \thead{$n_{kv-\text{heads}}$}   & \thead{$n_\text{ctx}$ \\ (pre-training)} & \thead{$d_\text{model}$} & \thead{$d_\text{ff}$} \\
		\midrule
		ChemFM-1B & $970$M & $22$ & $32$ & $4$ & $512$ & $2048$ & $5632$ \\
		ChemFM-3B & $3.0$B & $30$ & $48$ & $4$ & $512$ & $3072$ & $8640$ \\
		\midrule
		ChemFM-10M & $9.8$M & $3$ & $8$ & $8$ & $512$ & $512$ & $1408$ \\
		ChemFM-20M & $20.3$M & $4$ & $10$ & $10$ & $512$ & $640$ & $1760$ \\
		ChemFM-30M & $29,2$M & $4$ & $12$ & $12$ & $512$ & $768$ & $2112$ \\
		ChemFM-40M & $39.6$M & $4$ & $14$ & $14$ & $512$ & $896$ & $2464$ \\
		ChemFM-50M & $49.5$M & $5$ & $14$ & $14$ & $512$ & $896$ & $2464$ \\
		ChemFM-60M & $56.8$M & $5$ & $15$ & $15$ & $512$ & $960$ & $2640$ \\
		ChemFM-100M & $97.9$M & $6$ & $18$ & $18$ & $512$ & $1152$ & $3168$ \\
		ChemFM-200M & $201.1$M & $10$ & $20$ & $20$ & $512$ & $1280$ & $3520$ \\
		\botrule
	\end{tabular}
	\footnotetext{
		ChemFM-1B and ChemFM-3B are the primary models, while ChemFM-10M to ChemFM-200M are the models used for the scaling experiments.
		%
		$n_\text{params}$ is the actual number of non-embedding trainable parameters, $n_\text{layers}$ is the number of hidden layers in the Transformer decoder, $n_\text{heads}$ is the number of attention heads for each attention layer in the Transformer decoder, 
		$n_{kv-\text{heads}}$ is the number of key-value pairs for grouped query attention\cite{gqa},	
		$n_\text{ctx}$ is the context length, $d_\text{model}$ is the dimension of the hidden representations, and $d_\text{ff}$ is the dimension of the MLP representations. %
		It should be noted that, for training efficiency, the context lengths during fine-tuning may differ from those used in pre-training, depending on the maximum length of the dataset.}
\end{table}


==> tables/pretrain_generations.tex <==
\begin{table}[hp]
	%\caption{\textbf{Architectures of the ChemFM models.}} 	\label{table:model_architecture}
	\begin{tabular}{lccccc}
		\toprule
		\thead{Model} &
		\thead{Valid} & \thead{Unique} & \thead{Novelty}  & \thead{IntDiv$_1$/IntDiv$_2$} & \thead{KLDiv} \\
		\midrule
		ChemFM-1B & $0.995$ & $1.000$ & $0.577$ & $0.895$ &  $0.993$ \\
		ChemFM-3B & $0.996$ & $1.000$ & $0.558$ & $0.896$ & $0.993$ \\
		\botrule
	\end{tabular}
\end{table}


==> tables/results_MolGen.tex <==
\begin{table*}[!h]
	\caption{\textbf{Performance comparison on benchmarks for molecule generations.} }	\label{table:rst_prop_prediction}
	\begin{tabular}{cccccc}
		\toprule
		\thead{Condition types} & \thead{Property} & \thead{Validity} & \thead{Unique} & \thead{MAD} & \thead{SD} \\ 
		\midrule
		\multirow{16}{*}{Property} &	\multirow{2}{*}{logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{TPSA}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{SAS}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                            \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{QED}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                            \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{SAS + logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                            \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{SAS + TPSA}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                            \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{TPSA + logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                            \cmidrule(r){2-6}
		                           &	\multirow{2}{*}{TPSA + logP + SAS}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		                           &                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\midrule
		\multirow{2}{*}{Scaffold}&	\multirow{2}{*}{N/A}              & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
							     &                                   & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\midrule
		\multirow{16}{*}{Scaffold + Property}&	\multirow{2}{*}{logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{TPSA}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{SAS}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{QED}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{SAS + logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{SAS + TPSA}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{TPSA + logP}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\cmidrule(r){2-6}
		&	\multirow{2}{*}{TPSA + logP + SAS}            & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		&                                     & $0.0$            &  $0.0$         &  $0.0$             &   $0.0$ \\
		\botrule
\end{tabular}
\end{table*}


==> tables/results_PropPred_Admet_from_sweep.tex <==
%\begin{table}[!ht]
	%\centering	
\noindent
\begin{minipage}{1.0\textwidth}
	%\tablebodyfont
	\captionof{table}{\textbf{Performance comparison on 22 ADMET benchmark datasets with the previous best models for each molecular property prediction task.}} 		\label{table:rst_prop_prediction_admet}
		\footnotesize
		\begin{tabular}{lllll}
			\toprule
			Category & Dataset & Task metric & Previous best
			%& \thead{Previous second best} 
			& ChemFM \\ 
			\midrule
			Absorption & Caco2\_Wang & MAE $\downarrow$ & $0.330\pm0.024$@Chemprop-RDKit\cite{chemprop-rdkit} 
			%& $0.344\pm0.015$@Chemprop\cite{dmpnn} 
			& $\mathbf{0.325}^\star\pm0.022$ \\ 
			& Bioavailability\_Ma & ROC-AUC $\uparrow$ & $0.672\pm0.021$@DeepPurpose\cite{deeppurpose} 
			%& $0.671\pm0.026$ 
			& $\mathbf{0.715}\pm0.011$ \\ 
			& Lipophilicity\_AstraZeneca & MAE $\downarrow$ & $0.467\pm0.006$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.459}\pm0.007$\\ 
			& Solubility\_AqSolDB & MAE $\downarrow$ & $0.761\pm0.025$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.721}\pm0.011$\\ 
			& HIA\_Hou & ROC-AUC $\uparrow$ &$0.981\pm0.002$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.985}^\star\pm0.006$\\ 
			& Pgp\_Broccatelli & ROC-AUC $\uparrow$ & $0.929\pm0.006$@AttrMasking\cite{attrmasking} & $\mathbf{0.931}\pm0.003$ \\
			\midrule
			Distribution & BBB\_Martins & ROC-AUC $\uparrow$ & $0.897\pm0.004$@ContextPred\cite{attrmasking} & $\mathbf{0.909}\pm0.011$\\ 
			& PPBR\_AZ & MAE $\downarrow$ & $7.788\pm0.210$@Chemprop\cite{dmpnn} & $\mathbf{7.570}\pm0.094$\\ 
			& VDss\_Lombardo & Spearman $\uparrow$ & $0.561\pm0.025$@DeepPurpose\cite{deeppurpose} & $\mathbf{0.656}\pm0.024$\\
			\midrule 
			Metabolism & CYP2C9\_Veith & PRC-AUC $\uparrow$ & $0.777\pm0.003$@Chemprop-RDKit\cite{chemprop-rdkit}& $\mathbf{0.788}\pm0.005$ \\ 
			& CYP2D6\_Veith & PRC-AUC $\uparrow$ & $0.673\pm0.007$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.702}\pm0.005$\\ 
			& CYP3A4\_Veith & PRC-AUC $\uparrow$ & $0.876\pm0.003$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.877}\pm0.002$\\ 
			& CYP2C9\_Substrate\_CarbonMangels & PRC-AUC $\uparrow$ & $0.400\pm0.008$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.414}\pm0.027$ \\ 
			& CYP2D6\_Substrate\_CarbonMangels & PRC-AUC $\uparrow$ & $0.686\pm0.031$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.739}\pm0.024$\\   
			& CYP3A4\_Substrate\_CarbonMangels & ROC-AUC $\uparrow$ & $0.619\pm0.030$@Chemprop-RDKit\cite{chemprop-rdkit} & 
			$\mathbf{0.685}\pm0.011$
			\\
			\midrule
			Excretion &Half\_Life\_Obach & Spearman $\uparrow$ &$0.329\pm0.083$@DeepPurpose\cite{deeppurpose}  & $\mathbf{0.554}\pm0.023$\\ 
			& Clearance\_Hepatocyte\_AZ & Spearman $\uparrow$ & $0.439\pm0.026$@ContextPred\cite{attrmasking} & $\mathbf{0.496}\pm0.030$\\ 
			& Clearance\_Microsome\_AZ & Spearman $\uparrow$ & $0.599\pm0.025$@Chemprop-RDKit\cite{chemprop-rdkit} & 
			$\mathbf{0.610}\pm0.017$
			\\
			\midrule
			Toxicity & LD50\_Zhu & MAE $\downarrow$ & $0.606\pm0.024$@Chemprop\cite{dmpnn} & $\mathbf{0.545}\pm0.013$\\ 
			& hERG & ROC-AUC $\uparrow$ & $0.841\pm0.020$@DeepPurpose\cite{deeppurpose} & $\mathbf{0.848}\pm0.009$\\ 
			& AMES & ROC-AUC $\uparrow$ & $0.850\pm0.004$@Chemprop-RDKit\cite{chemprop-rdkit} & $\mathbf{0.854}\pm0.007$ \\ 
			& DILI & ROC-AUC $\uparrow$ & $0.919\pm0.008$@ContextPred\cite{attrmasking} & $\mathbf{0.920}\pm0.012$\\ 
%	
%				Pharmacokinetic & BBBP &  ROC-AUC $\uparrow$ & Scaffold & $0.729$ (KernelSVM) & $0.738$ & $0.739$ & $0.745/\mathbf{0.751}$\\
%				\midrule
%				\multirow{2}{*} {Bioactivity} & BACE & ROC-AUC $\uparrow$ & Scaffold & $0.867$ (RF)& N/A & $0.835$ & $0.827/\mathbf{0.869}$ \\
%				%& BACE & ROC-AUC $\uparrow$ & Scaffold & $0.690$ & $0.738$ & $0.739$ & $0.745/\mathbf{0.751}$ \\
%				& HIV & ROC-AUC $\uparrow$ & Scaffold & $0.792$ (KernelSVM) & $0.776$ & $0.777$ & $0.785/\mathbf{0.807}$ \\
%				\midrule
%				\multirow{3}{*} {Toxicity} & Tox21 & ROC-AUC $\uparrow$ & Random & $0.829$ (GC) & $0.851$ & $0.845$ & $0.862/\mathbf{0.863}$ \\
%				& SIDER & ROC-AUC $\uparrow$ & Random & $0.684$ (RF) & $0.676$ & $0.680$ & $0.702/\mathbf{0.709}$ \\
%				& ClinTox & ROC-AUC $\uparrow$ & Random & $0.832$ (Weave) & $0.864$ & $0.888$ & $0.899/\mathbf{0.918}$ \\
%				\midrule
%				\multirow{3}{*} {Physicochemical} & ESOL & RMSE $\downarrow$ & Random & $0.580$ (MPNN) & $0.555$ & $0.575$ & $0.529/\mathbf{0.516}$ \\
%				& FreeSolv & RMSE $\downarrow$ & Random & $1.150$ (MPNN) & $1.075$ & $1.155$ & $0.906/\mathbf{0.830}$ \\
%				& Lipophilicity & RMSE $\downarrow$ & Random & $0.655$ (GC) & $0.555$ & $0.625$ & $0.547/\mathbf{0.545}$ \\
%				\midrule
%				\makecell{Molecular binding} & PDBbind-F & RMSE $\downarrow$ & Time & $1.250$ (RF) & $1.391$ & $0.721$ & $0.700/\mathbf{0.697}$ \\
				%& FreeSolv & RMSE $\downarrow$ & Random & $1.150$ & $1.075$ & $1.155$ & $0.906/\mathbf{0.830}$ \\
				%& Lipop & RMSE $\downarrow$ & Random & $0.655$ & $0.555$ & $0.625$ & $0.547/\mathbf{0.545}$ \\
				%		\multirow{6}{*}{\makecell{Classification \\ (ROC-AUC $\uparrow$)} } %\\ Metric: ROC-AUC $\uparrow$ }
			%		& BBBP & Scaffold & $0.944$ @PanGu\cite{pangu} & $0.940$ @GROVER\cite{grover} & $0.956$ \\ 
			%		& Tox21 &  Random & $0.858$ @CLM\cite{CLM} & $0.858$ @AttenFP\cite{attentiveFP} & $0.806$ \\ 
			%		& ClinTox &   Random & $0.940$ @AttenFP\cite{attentiveFP} & $0.896$ @PanGu\cite{pangu}& $0.980$ \\ 
			%		& HIV &  Scaffold & $0.832$ @AttenFP\cite{attentiveFP} & $0.813$ @CLM\cite{CLM} & $0.783$ \\ 
			%		& BACE & Scaffold & $0.917$ @PanGu\cite{pangu} & $0.894$ @GROVER\cite{grover} & $0.928$ \\
			%		& SIDER &  Random & $0.723$ @SELFormer\cite{selformer} & $0.680$ @MMNB\cite{MMNB} & $0.938$ \\
			%		\midrule
			%		\multirow{4}{*}{\makecell{Regression \\ (RMSE $\downarrow$)} } %\\ Metric: RMSE $\downarrow$ }
		%		& ESOL & Random & $0.380$ @SELFormer\cite{selformer}  & $0.531$ @MolBERT\cite{molbert} & $0.332$ \\ 
		%		& FreeSolv &  Random & $0.736$ @AttenFP\cite{attentiveFP} & $0.941$ @MolBERT\cite{molbert} & $0.041$ \\ 
		%		& Lipophilicity &   Random & $0.561$ @MolBERT\cite{molbert} & $0.578$ @AttenFP\cite{attentiveFP} & $0.431$ \\ 
		%		& PDBbind &  Random & $0.721$ @MMNB\cite{MMNB} & $1.397$ @D-MPNN\cite{dmpnn}  & $1.155$ \\ 	
		\botrule
	\end{tabular}
	\captionof*{tabledescription}{	We use the default metrics and scaffold split methods, with the data pre-split by the benchmark.
		%
		\textbf{Bold} values indicate the best-performing models. 
		%
		Evaluation metrics include ROC-AUC, PRC-AUC, MAE, and Spearman’s rank correlation coefficient, with an upward arrow ($\uparrow$) indicating that higher values are better and a downward arrow ($\downarrow$) indicating that lower values are better. 
		%
		All ChemFM results are fine-tuned from the ChemFM-3B model, except those marked with a $\star$, which are fine-tuned from the ChemFM-1B model.}
\end{minipage}
%\end{table}


==> tables/results_cond_mol_generation_scaffold_2d.tex <==
\begin{table}\ContinuedFloat
	\centering
	\footnotesize
	\caption{\textbf{Performance comparison on standard benchmarks for conditional molecule generation.}}
	\begin{tabular}{ccccccccc}
		\toprule
		Property & Scaffold  & Model &\makecell[c]{Generation \\ count} & \makecell[c]{Valid \\ molecules $\uparrow$} & \makecell[c]{Unique \\ molecules $\uparrow$} & \makecell[c]{Novel \\ molecules $\uparrow$} & \makecell[c]{Same scaffold \\ molecules $\uparrow$} & \makecell[c]{MAD $\downarrow$}  \\
		\midrule   
		\multirow{15}{*}{\shortstack{TPSA + \\ $\log$P}} 
		& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{38440}$ & $\num{8919}$ & $\num{8919}$ & $\num{8919}$ & $\num{3.266}/\num{0.182}$\\
		&                      & ChemFM & $\num{40000}$ & $\num{38529}$ & $\num{21348}$ & $\num{21320}$ & $\num{21344}$ & $\num{3.567}/\num{0.183}$\\
		\cmidrule{2-9}
		& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{33172}$ & $\num{16609}$ & $\num{16609}$ & $\num{16578}$ & $\num{4.195}/\num{0.196}$\\
		&                      & ChemFM & $\num{40000}$ & $\num{37005}$ & $\num{30376}$ & $\num{30375}$ & $\num{30018}$ & $\num{2.797}/\num{0.153}$\\
		\cmidrule{2-9}
		& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{38190}$ & $\num{13901}$ & $\num{13901}$ & $\num{13881}$ & $\num{3.733}/\num{0.159}$\\
		&                      & ChemFM & $\num{40000}$ & $\num{38732}$ & $\num{22421}$ & $\num{22421}$ & $\num{22409}$ & $\num{2.931}/\num{0.155}$\\
		\cmidrule{2-9}
		& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{36010}$ & $\num{11104}$ & $\num{11104}$ & $\num{11102}$ & $\num{4.113}/\num{0.165}$\\
		&                      & ChemFM & $\num{40000}$ & $\num{37689}$ & $\num{23576}$ & $\num{23547}$ & $\num{23527}$ & $\num{3.439}/\num{0.204}$\\
		\cmidrule{2-9}
		& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{36122}$ & $\num{3966}$ & $\num{3965}$ & $\num{3942}$ & $\num{6.028}/\num{0.374}$\\
		&                      & ChemFM & $\num{40000}$ & $\num{39081}$ & $\num{14444}$ & $\num{14441}$ & $\num{14366}$ & $\num{3.881}/\num{0.172}$\\
		\cmidrule{2-9}
		& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{181934}$ & $\num{54499}$ & $\num{54498}$ & $\num{54422}$ & $\num{4.042}/\num{0.191}$\\
		&                      & ChemFM & $\num{200000}$ & $\num{191036}$ & $\num{112165}$ & $\num{112104}$ & $\num{111664}$ & $\num{3.245}/\num{0.173}$\\
		\midrule
		\multirow{15}{*}{\shortstack{SAS + \\ $\log$P}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{36497}$ & $\num{11866}$ & $\num{11866}$ & $\num{11859}$ & $\num{0.185}/\num{0.301}$\\
&                      & ChemFM & $\num{40000}$ & $\num{34847}$ & $\num{24198}$ & $\num{24178}$ & $\num{24163}$ & $\num{0.147}/\num{0.277}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{30249}$ & $\num{10962}$ & $\num{10962}$ & $\num{10958}$ & $\num{0.156}/\num{0.191}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36576}$ & $\num{19477}$ & $\num{19471}$ & $\num{19297}$ & $\num{0.207}/\num{0.215}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{36784}$ & $\num{12745}$ & $\num{12745}$ & $\num{12734}$ & $\num{0.167}/\num{0.199}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38596}$ & $\num{21356}$ & $\num{21355}$ & $\num{21322}$ & $\num{0.198}/\num{0.256}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{37290}$ & $\num{11616}$ & $\num{11616}$ & $\num{11613}$ & $\num{0.177}/\num{0.246}$\\
&                      & ChemFM & $\num{40000}$ & $\num{39119}$ & $\num{23549}$ & $\num{23495}$ & $\num{23522}$ & $\num{0.166}/\num{0.337}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{39243}$ & $\num{4361}$ & $\num{4361}$ & $\num{4262}$ & $\num{0.174}/\num{0.282}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38430}$ & $\num{15557}$ & $\num{15553}$ & $\num{15476}$ & $\num{0.214}/\num{0.296}$\\
\cmidrule{2-9}
& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{180063}$ & $\num{51550}$ & $\num{51550}$ & $\num{51426}$ & $\num{0.172}/\num{0.238}$\\
&                      & ChemFM & $\num{200000}$ & $\num{187568}$ & $\num{104137}$ & $\num{104052}$ & $\num{103780}$ & $\num{0.183}/\num{0.278}$\\
		\midrule
		\multirow{15}{*}{\shortstack{TPSA + \\ SAS}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{37901}$ & $\num{16217}$ & $\num{16217}$ & $\num{16214}$ & $\num{4.110}/\num{0.222}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36655}$ & $\num{26041}$ & $\num{26025}$ & $\num{26000}$ & $\num{5.042}/\num{0.158}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{32343}$ & $\num{12808}$ & $\num{12808}$ & $\num{12744}$ & $\num{4.037}/\num{0.183}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36298}$ & $\num{20567}$ & $\num{20560}$ & $\num{20366}$ & $\num{3.988}/\num{0.222}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{31731}$ & $\num{13522}$ & $\num{13522}$ & $\num{13512}$ & $\num{4.789}/\num{0.186}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38596}$ & $\num{21370}$ & $\num{21366}$ & $\num{21318}$ & $\num{4.729}/\num{0.202}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{35947}$ & $\num{13793}$ & $\num{13793}$ & $\num{13793}$ & $\num{4.795}/\num{0.226}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38923}$ & $\num{23481}$ & $\num{23444}$ & $\num{23440}$ & $\num{4.756}/\num{0.166}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{39196}$ & $\num{5170}$ & $\num{5170}$ & $\num{5120}$ & $\num{4.561}/\num{0.208}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38562}$ & $\num{13473}$ & $\num{13471}$ & $\num{13424}$ & $\num{5.855}/\num{0.217}$\\
\cmidrule{2-9}
& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{177118}$ & $\num{61510}$ & $\num{61510}$ & $\num{61383}$ & $\num{4.435}/\num{0.206}$\\
&                      & ChemFM & $\num{200000}$ & $\num{189034}$ & $\num{104932}$ & $\num{104866}$ & $\num{104548}$ & $\num{4.812}/\num{0.189}$\\
\midrule
		\multirow{15}{*}{\shortstack{TPSA + \\ $\log$P + \\ SAS}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{80000}$ & $\num{66217}$ & $\num{14699}$ & $\num{14699}$ & $\num{14699}$ & $\num{5.658}/\num{0.356}/\num{0.335}$\\
&                      & ChemFM & $\num{80000}$ & $\num{69595}$ & $\num{40254}$ & $\num{40227}$ & $\num{40244}$ & $\num{7.246}/\num{0.673}/\num{0.260}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{80000}$ & $\num{63655}$ & $\num{17279}$ & $\num{17279}$ & $\num{17257}$ & $\num{4.592}/\num{0.237}/\num{0.206}$\\
&                      & ChemFM & $\num{80000}$ & $\num{66662}$ & $\num{34500}$ & $\num{34494}$ & $\num{34058}$ & $\num{4.001}/\num{0.241}/\num{0.236}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{80000}$ & $\num{59363}$ & $\num{16086}$ & $\num{16086}$ & $\num{16068}$ & $\num{5.793}/\num{0.307}/\num{0.271}$\\
&                      & ChemFM & $\num{80000}$ & $\num{71915}$ & $\num{31335}$ & $\num{31333}$ & $\num{31204}$ & $\num{5.371}/\num{0.350}/\num{0.231}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{80000}$ & $\num{50119}$ & $\num{12081}$ & $\num{12081}$ & $\num{12080}$ & $\num{5.577}/\num{0.312}/\num{0.320}$\\
&                      & ChemFM & $\num{80000}$ & $\num{74396}$ & $\num{30787}$ & $\num{30720}$ & $\num{30609}$ & $\num{6.659}/\num{0.634}/\num{0.254}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{80000}$ & $\num{74433}$ & $\num{7228}$ & $\num{7228}$ & $\num{7111}$ & $\num{6.709}/\num{0.353}/\num{0.255}$\\
&                      & ChemFM & $\num{80000}$ & $\num{71057}$ & $\num{23298}$ & $\num{23294}$ & $\num{22858}$ & $\num{7.595}/\num{0.493}/\num{0.288}$\\
\cmidrule{2-9}
& \multirow{2}{*}{In total} & MolGPT & $\num{400000}$ & $\num{313787}$ & $\num{67373}$ & $\num{67373}$ & $\num{67215}$ & $\num{5.515}/\num{0.305}/\num{0.275}$\\
&                      & ChemFM & $\num{400000}$ & $\num{353625}$ & $\num{160174}$ & $\num{160068}$ & $\num{158973}$ & $\num{6.118}/\num{0.483}/\num{0.252}$\\			
		\bottomrule
	\end{tabular}	
	\tablebodyfont
	\footnotetext{
		The molecules are generated conditioned on desired scaffold and property values. We compare the generation performance between ChemFM-3B  and  MolGPT\cite{molgpt}, evaluating the validity, uniqueness, mean average deviation (MAD) and standard deviation (SD) of the generated molecules.
		(a) O$=$C
		
	}
\end{table}

==> tables/results_cond_mol_generation_scaffold_old.tex <==
%\noindent
\noindent
%\begin{minipage}{1.0\textwidth}
{
\footnotesize
\begin{longtable}[l]{ccccccccc}
	%\centering
	%\begin{tabular}{ccccccccc}
	\caption{\textbf{Performance comparison for conditional molecular generation.}}
	\label{table:rst_conditional_molecular_generation}\\\toprule
	Property & Scaffold  & Model &\makecell[c]{Generation \\ count} & \makecell[c]{Valid \\ molecules $\uparrow$} & \makecell[c]{Unique \\ molecules $\uparrow$} & \makecell[c]{Novel \\ molecules $\uparrow$} & \makecell[c]{Same scaffold \\ molecules $\uparrow$} & \makecell[c]{MAD $\downarrow$}  \\
	\midrule 	
	\endfirsthead
	%\multicolumn{9}{c}%
	%{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
	\caption*{\textbf{\textbf{\tablename\ \thetable{} Continued:} Performance comparison on standard benchmarks for conditional molecular generation.}}\\\toprule
	Property & Scaffold  & Model &\makecell[c]{Generation \\ count} & \makecell[c]{Valid \\ molecules $\uparrow$} & \makecell[c]{Unique \\ molecules $\uparrow$} & \makecell[c]{Novel \\ molecules $\uparrow$} & \makecell[c]{Same scaffold \\ molecules $\uparrow$} & \makecell[c]{MAD $\downarrow$}  \\
	\midrule 
	%\label{table:rst_conditional_molecular_generation}\\
	\endhead	
	 \multicolumn{9}{r}{{Continued on next page}} \\ 
	\endfoot
	\bottomrule
	\endlastfoot	
	%\toprule
%	Property & Scaffold  & Model &\makecell[c]{Generation \\ count} & \makecell[c]{Valid \\ molecules $\uparrow$} & \makecell[c]{Unique \\ molecules $\uparrow$} & \makecell[c]{Novel \\ molecules $\uparrow$} & \makecell[c]{Same scaffold \\ molecules $\uparrow$} & \makecell[c]{MAD $\downarrow$}  \\	
%	\midrule  
	\multirow{13}{*}{logP} & \multirow{2}{*}{(a)} &  MolGPT & $\num{30000}$ & $\num{29679}$ & $\num{7132}$ & $\num{7132}$ & $\num{7132}$ & $0.119$  \\
	                          &                  &  ChemFM & $\num{30000}$ & $\num{29450}$ & $\num{16484}$ & $\num{16447}$ & $\num{16483}$ & $0.160$ \\
	                          \cmidrule{2-9}
	                          & \multirow{2}{*}{(b)} &  MolGPT &  $\num{30000}$ & $\num{29666}$ & $\num{2334}$ & $\num{2334}$ & $\num{2328}$ & $0.160$ \\
	                          &                  &  ChemFM & $\num{30000}$ & $\num{29545}$ & $\num{7237}$ & $\num{7232}$ & $\num{7231}$ & $0.177$ \\
	                          \cmidrule{2-9}
	                          & \multirow{2}{*}{(c)} &  MolGPT &  $\num{30000}$ & $\num{28536}$ & $\num{10537}$ & $\num{10537}$ & $\num{10531}$ & $0.136$ \\
	                          &                  &  ChemFM & $\num{30000}$ & $\num{29501}$ & $\num{19156}$ & $\num{19153}$ & $\num{19146}$ & $0.136$\\
	                          \cmidrule{2-9}
	                          & \multirow{2}{*}{(d)} &  MolGPT &  $\num{30000}$ & $\num{29643}$ & $\num{8886}$ & $\num{8886}$ & $\num{8885}$ & $0.146$ \\
	                          &                  &  ChemFM & $\num{30000}$ & $\num{29731}$ & $\num{19536}$ & $\num{19474}$ & $\num{19532}$ & $0.182$\\
	                          \cmidrule{2-9}
	                          & \multirow{2}{*}{(e)} &  MolGPT &  $\num{30000}$ & $\num{26880}$ & $\num{15669}$ & $\num{15669}$ & $\num{15669}$ & $0.134$ \\
	                          &                  &  ChemFM & $\num{30000}$ & $\num{27900}$ & $\num{23405}$ & $\num{23395}$ & $\num{23244}$ & $0.141$\\
	                        %  \cmidrule{2-9}
	                       %   & \multirow{2}{*}{In total} &  MolGPT &  $\num{150000}$ & $\num{144404}$ & $\num{44558}$ & $\num{44558}$ & $\num{44545}$ & $0.136$ \\
	                       %   &                  &  ChemFM & $\num{150000}$ & $\num{146127}$ & $\num{85818}$ & $\num{85701}$ & $\num{85636}$ & $0.156$\\
	\midrule   
	\multirow{13}{*}{SAS} 
	& \multirow{2}{*}{(a)} & MolGPT & $\num{30000}$ & $\num{29253}$ & $\num{13663}$ & $\num{13663}$ & $\num{13663}$ & $\num{0.141}$  \\
	&                      & ChemFM & $\num{30000}$ & $\num{27697}$ & $\num{22263}$ & $\num{22229}$ & $\num{22237}$ & $\num{0.135}$  \\
	\cmidrule{2-9}
	& \multirow{2}{*}{(b)} & MolGPT & $\num{30000}$ & $\num{26719}$ & $\num{11846}$ & $\num{11846}$ & $\num{11843}$ & $\num{0.142}$  \\
	&                      & ChemFM & $\num{30000}$ & $\num{28053}$ & $\num{18590}$ & $\num{18580}$ & $\num{18415}$ & $\num{0.177}$  \\
	\cmidrule{2-9}
	& \multirow{2}{*}{(c)} & MolGPT & $\num{30000}$ & $\num{25269}$ & $\num{10803}$ & $\num{10803}$ & $\num{10791}$ & $\num{0.149}$  \\
	&                      & ChemFM & $\num{30000}$ & $\num{29229}$ & $\num{21177}$ & $\num{21176}$ & $\num{21141}$ & $\num{0.163}$  \\
	\cmidrule{2-9}
	& \multirow{2}{*}{(d)} & MolGPT & $\num{30000}$ & $\num{29011}$ & $\num{12253}$ & $\num{12253}$ & $\num{12253}$ & $\num{0.180}$  \\
	&                      & ChemFM & $\num{30000}$ & $\num{29490}$ & $\num{24398}$ & $\num{24323}$ & $\num{24392}$ & $\num{0.137}$  \\
	\cmidrule{2-9}
	& \multirow{2}{*}{(e)} & MolGPT & $\num{30000}$ & $\num{28540}$ & $\num{4087}$ & $\num{4087}$ & $\num{4065}$ & $\num{0.168}$  \\
	&                      & ChemFM & $\num{30000}$ & $\num{29487}$ & $\num{10484}$ & $\num{10478}$ & $\num{10464}$ & $\num{0.208}$ \\
	%\cmidrule{2-9}
	%& \multirow{2}{*}{In total} & MolGPT & $\num{150000}$ & $\num{138792}$ & $\num{52652}$ & $\num{52652}$ & $\num{52615}$ & $\num{0.154}$  \\
	%&                      & ChemFM & $\num{150000}$ & $\num{143956}$ & $\num{96912}$ & $\num{96786}$ & $\num{96649}$ & $\num{0.157}$  \\
	\midrule
	\multirow{13}{*}{TPSA} 
	& \multirow{2}{*}{(a)} & MolGPT & $\num{30000}$ & $\num{29809}$ & $\num{8134}$ & $\num{8134}$ & $\num{8132}$ & $\num{2.454}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29673}$ & $\num{15834}$ & $\num{15791}$ & $\num{15832}$ & $\num{3.084}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(b)} & MolGPT & $\num{30000}$ & $\num{26509}$ & $\num{14519}$ & $\num{14519}$ & $\num{14518}$ & $\num{3.112}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{28083}$ & $\num{21690}$ & $\num{21681}$ & $\num{21553}$ & $\num{3.063}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(c)} & MolGPT & $\num{30000}$ & $\num{29522}$ & $\num{10240}$ & $\num{10240}$ & $\num{10240}$ & $\num{2.674}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29535}$ & $\num{18101}$ & $\num{18100}$ & $\num{18090}$ & $\num{2.903}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(d)} & MolGPT & $\num{30000}$ & $\num{29655}$ & $\num{10264}$ & $\num{10264}$ & $\num{10263}$ & $\num{3.040}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29787}$ & $\num{20182}$ & $\num{20115}$ & $\num{20172}$ & $\num{3.097}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(e)} & MolGPT & $\num{30000}$ & $\num{28716}$ & $\num{1873}$ & $\num{1873}$ & $\num{1867}$ & $\num{5.343}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29613}$ & $\num{8686}$ & $\num{8679}$ & $\num{8683}$ & $\num{4.594}$\\
	%\cmidrule{2-9}
	%& \multirow{2}{*}{In total} & MolGPT & $\num{150000}$ & $\num{144211}$ & $\num{45030}$ & $\num{45030}$ & $\num{45020}$ & $\num{2.970}$\\
	%&                      & ChemFM & $\num{150000}$ & $\num{146691}$ & $\num{84493}$ & $\num{84366}$ & $\num{84330}$ & $\num{3.198}$\\
	\midrule
	\multirow{13}{*}{QED} 
	& \multirow{2}{*}{(a)} & MolGPT & $\num{30000}$ & $\num{29618}$ & $\num{12931}$ & $\num{12931}$ & $\num{12931}$ & $\num{0.050}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29196}$ & $\num{22186}$ & $\num{22127}$ & $\num{22185}$ & $\num{0.042}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(b)} & MolGPT & $\num{30000}$ & $\num{25516}$ & $\num{15659}$ & $\num{15659}$ & $\num{15646}$ & $\num{0.046}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{27894}$ & $\num{22763}$ & $\num{22751}$ & $\num{22612}$ & $\num{0.048}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(c)} & MolGPT & $\num{30000}$ & $\num{29055}$ & $\num{13108}$ & $\num{13108}$ & $\num{13105}$ & $\num{0.041}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29173}$ & $\num{20427}$ & $\num{20422}$ & $\num{20406}$ & $\num{0.049}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(d)} & MolGPT & $\num{30000}$ & $\num{29812}$ & $\num{12978}$ & $\num{12978}$ & $\num{12978}$ & $\num{0.062}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29823}$ & $\num{20354}$ & $\num{20243}$ & $\num{20349}$ & $\num{0.049}$\\
	\cmidrule{2-9}
	& \multirow{2}{*}{(e)} & MolGPT & $\num{30000}$ & $\num{27457}$ & $\num{2918}$ & $\num{2918}$ & $\num{2909}$ & $\num{0.115}$\\
	&                      & ChemFM & $\num{30000}$ & $\num{29557}$ & $\num{10855}$ & $\num{10848}$ & $\num{10834}$ & $\num{0.061}$\\
	%\cmidrule{2-9}
	%& \multirow{2}{*}{In total} & MolGPT & $\num{150000}$ & $\num{141458}$ & $\num{57594}$ & $\num{57594}$ & $\num{57569}$ & $\num{0.053}$\\
	%&                      & ChemFM & $\num{150000}$ & $\num{145643}$ & $\num{96585}$ & $\num{96391}$ & $\num{96386}$ & $\num{0.048}$\\	
	\midrule  
\multirow{13}{*}{\shortstack{TPSA + \\ $\log$P}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{38440}$ & $\num{8919}$ & $\num{8919}$ & $\num{8919}$ & $\num{3.266}/\num{0.182}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38529}$ & $\num{21348}$ & $\num{21320}$ & $\num{21344}$ & $\num{3.567}/\num{0.183}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{33172}$ & $\num{16609}$ & $\num{16609}$ & $\num{16578}$ & $\num{4.195}/\num{0.196}$\\
&                      & ChemFM & $\num{40000}$ & $\num{37005}$ & $\num{30376}$ & $\num{30375}$ & $\num{30018}$ & $\num{2.797}/\num{0.153}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{38190}$ & $\num{13901}$ & $\num{13901}$ & $\num{13881}$ & $\num{3.733}/\num{0.159}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38732}$ & $\num{22421}$ & $\num{22421}$ & $\num{22409}$ & $\num{2.931}/\num{0.155}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{36010}$ & $\num{11104}$ & $\num{11104}$ & $\num{11102}$ & $\num{4.113}/\num{0.165}$\\
&                      & ChemFM & $\num{40000}$ & $\num{37689}$ & $\num{23576}$ & $\num{23547}$ & $\num{23527}$ & $\num{3.439}/\num{0.204}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{36122}$ & $\num{3966}$ & $\num{3965}$ & $\num{3942}$ & $\num{6.028}/\num{0.374}$\\
&                      & ChemFM & $\num{40000}$ & $\num{39081}$ & $\num{14444}$ & $\num{14441}$ & $\num{14366}$ & $\num{3.881}/\num{0.172}$\\
%\cmidrule{2-9}
%& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{181934}$ & $\num{54499}$ & $\num{54498}$ & $\num{54422}$ & $\num{4.042}/\num{0.191}$\\
%&                      & ChemFM & $\num{200000}$ & $\num{191036}$ & $\num{112165}$ & $\num{112104}$ & $\num{111664}$ & $\num{3.245}/\num{0.173}$\\
\midrule
\multirow{13}{*}{\shortstack{SAS + \\ $\log$P}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{36497}$ & $\num{11866}$ & $\num{11866}$ & $\num{11859}$ & $\num{0.185}/\num{0.301}$\\
&                      & ChemFM & $\num{40000}$ & $\num{34847}$ & $\num{24198}$ & $\num{24178}$ & $\num{24163}$ & $\num{0.147}/\num{0.277}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{30249}$ & $\num{10962}$ & $\num{10962}$ & $\num{10958}$ & $\num{0.156}/\num{0.191}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36576}$ & $\num{19477}$ & $\num{19471}$ & $\num{19297}$ & $\num{0.207}/\num{0.215}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{36784}$ & $\num{12745}$ & $\num{12745}$ & $\num{12734}$ & $\num{0.167}/\num{0.199}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38596}$ & $\num{21356}$ & $\num{21355}$ & $\num{21322}$ & $\num{0.198}/\num{0.256}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{37290}$ & $\num{11616}$ & $\num{11616}$ & $\num{11613}$ & $\num{0.177}/\num{0.246}$\\
&                      & ChemFM & $\num{40000}$ & $\num{39119}$ & $\num{23549}$ & $\num{23495}$ & $\num{23522}$ & $\num{0.166}/\num{0.337}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{39243}$ & $\num{4361}$ & $\num{4361}$ & $\num{4262}$ & $\num{0.174}/\num{0.282}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38430}$ & $\num{15557}$ & $\num{15553}$ & $\num{15476}$ & $\num{0.214}/\num{0.296}$\\
%\cmidrule{2-9}
%& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{180063}$ & $\num{51550}$ & $\num{51550}$ & $\num{51426}$ & $\num{0.172}/\num{0.238}$\\
%&                      & ChemFM & $\num{200000}$ & $\num{187568}$ & $\num{104137}$ & $\num{104052}$ & $\num{103780}$ & $\num{0.183}/\num{0.278}$\\
\midrule
\multirow{13}{*}{\shortstack{TPSA + \\ SAS}} 
& \multirow{2}{*}{(a)} & MolGPT & $\num{40000}$ & $\num{37901}$ & $\num{16217}$ & $\num{16217}$ & $\num{16214}$ & $\num{4.110}/\num{0.222}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36655}$ & $\num{26041}$ & $\num{26025}$ & $\num{26000}$ & $\num{5.042}/\num{0.158}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{40000}$ & $\num{32343}$ & $\num{12808}$ & $\num{12808}$ & $\num{12744}$ & $\num{4.037}/\num{0.183}$\\
&                      & ChemFM & $\num{40000}$ & $\num{36298}$ & $\num{20567}$ & $\num{20560}$ & $\num{20366}$ & $\num{3.988}/\num{0.222}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(c)} & MolGPT & $\num{40000}$ & $\num{31731}$ & $\num{13522}$ & $\num{13522}$ & $\num{13512}$ & $\num{4.789}/\num{0.186}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38596}$ & $\num{21370}$ & $\num{21366}$ & $\num{21318}$ & $\num{4.729}/\num{0.202}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(d)} & MolGPT & $\num{40000}$ & $\num{35947}$ & $\num{13793}$ & $\num{13793}$ & $\num{13793}$ & $\num{4.795}/\num{0.226}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38923}$ & $\num{23481}$ & $\num{23444}$ & $\num{23440}$ & $\num{4.756}/\num{0.166}$\\
\cmidrule{2-9}
& \multirow{2}{*}{(e)} & MolGPT & $\num{40000}$ & $\num{39196}$ & $\num{5170}$ & $\num{5170}$ & $\num{5120}$ & $\num{4.561}/\num{0.208}$\\
&                      & ChemFM & $\num{40000}$ & $\num{38562}$ & $\num{13473}$ & $\num{13471}$ & $\num{13424}$ & $\num{5.855}/\num{0.217}$\\
%\cmidrule{2-9}
%& \multirow{2}{*}{In total} & MolGPT & $\num{200000}$ & $\num{177118}$ & $\num{61510}$ & $\num{61510}$ & $\num{61383}$ & $\num{4.435}/\num{0.206}$\\
%&                      & ChemFM & $\num{200000}$ & $\num{189034}$ & $\num{104932}$ & $\num{104866}$ & $\num{104548}$ & $\num{4.812}/\num{0.189}$\\
\midrule
\multirow{20}{*}{\shortstack{TPSA + \\ $\log$P + \\ SAS}} 
& \multirow{3}{*}{(a)} & MolGPT & $\num{80000}$ & $\num{66217}$ & $\num{14699}$ & $\num{14699}$ & $\num{14699}$ & \makecell{$\num{5.658}/\num{0.356}/$\\$\num{0.335}$}\\
&                      & ChemFM & $\num{80000}$ & $\num{69595}$ & $\num{40254}$ & $\num{40227}$ & $\num{40244}$ & \makecell{$\num{7.246}/\num{0.673}/$\\$\num{0.260}$}\\
\cmidrule{2-9}
& \multirow{2}{*}{(b)} & MolGPT & $\num{80000}$ & $\num{63655}$ & $\num{17279}$ & $\num{17279}$ & $\num{17257}$ & \makecell{$\num{4.592}/\num{0.237}/$\\$\num{0.206}$}\\
&                      & ChemFM & $\num{80000}$ & $\num{66662}$ & $\num{34500}$ & $\num{34494}$ & $\num{34058}$ & \makecell{$\num{4.001}/\num{0.241}/$\\$\num{0.236}$}\\
\cmidrule{2-9}
& \multirow{3}{*}{(c)} & MolGPT & $\num{80000}$ & $\num{59363}$ & $\num{16086}$ & $\num{16086}$ & $\num{16068}$ & \makecell{$\num{5.793}/\num{0.307}/$\\$\num{0.271}$}\\
&                      & ChemFM & $\num{80000}$ & $\num{71915}$ & $\num{31335}$ & $\num{31333}$ & $\num{31204}$ & \makecell{$\num{5.371}/\num{0.350}/$\\$\num{0.231}$}\\
\cmidrule{2-9}
& \multirow{3}{*}{(d)} & MolGPT & $\num{80000}$ & $\num{50119}$ & $\num{12081}$ & $\num{12081}$ & $\num{12080}$ & \makecell{$\num{5.577}/\num{0.312}/$\\$\num{0.320}$}\\
&                      & ChemFM & $\num{80000}$ & $\num{74396}$ & $\num{30787}$ & $\num{30720}$ & $\num{30609}$ & \makecell{$\num{6.659}/\num{0.634}/$\\$\num{0.254}$}\\
\cmidrule{2-9}
& \multirow{3}{*}{(e)} & MolGPT & $\num{80000}$ & $\num{74433}$ & $\num{7228}$ & $\num{7228}$ & $\num{7111}$ & \makecell{$\num{6.709}/\num{0.353}/$\\$\num{0.255}$}\\
&                      & ChemFM & $\num{80000}$ & $\num{71057}$ & $\num{23298}$ & $\num{23294}$ & $\num{22858}$ & \makecell{$\num{7.595}/\num{0.493}/$\\$\num{0.288}$}\\
%\cmidrule{2-9}
%& \multirow{3}{*}{In total} & MolGPT & $\num{400000}$ & $\num{313787}$ & $\num{67373}$ & $\num{67373}$ & $\num{67215}$ & \makecell{$\num{5.515}/\num{0.305}/$\\$\num{0.275}$}\\
%&                      & ChemFM & $\num{400000}$ & $\num{353625}$ & $\num{160174}$ & $\num{160068}$ & $\num{158973}$ & \makecell{$\num{6.118}/\num{0.483}/$\\$\num{0.252}$}\\					
	%\bottomrule
%\end{tabular}	
	%\tablebodyfont
%	\footnotetext{
%		The molecules are generated conditioned on desired scaffold and property values. We compare the generation performance between ChemFM-3B  and  MolGPT\cite{molgpt}, evaluating the validity, uniqueness, mean average deviation (MAD) and standard deviation (SD) of the generated molecules.
%		(a) O$=$C	
%	}
\end{longtable}
\captionof*{tabledescription}{The molecules are generated conditioned on desired scaffold and property values. We compare the generation performance between ChemFM-3B  and  MolGPT\cite{molgpt}, evaluating the validity, uniqueness, mean average deviation (MAD) and standard deviation (SD) of the generated molecules.}
}
	%		(a) O$=$C	}
%\end{minipage}
